All two-loop scalar self-energies and tadpoles in general renormalisable field theories

We calculate the complete tadpoles and self-energies at the two-loop order for scalars in general renormalisable theories, a crucial component for calculating two-loop electroweak corrections to Higgs-boson masses or for any scalar beyond the Standard Model. We renormalise the amplitudes using mass-independent renormalisation schemes, based on both dimensional regularisation and dimensional reduction. The results are presented here in Feynman gauge, with expressions for all 121 self-energy and 25 tadpole diagrams given in terms of scalar and tensor integrals with the complete set of rules to reduce them to a minimal basis of scalar integrals for any physical kinematic configuration. In addition, we simplify the results to a set of only 16 tadpole and 58 self-energy topologies using relations in order to substitute the ghost and Goldstone-boson couplings that we derive. To facilitate their application, we also provide our results in electronic form as a new code TLDR. We test our results by applying them to the Standard Model and compare with analytic expressions in the literature.

==> TeX/Selfs/001.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSS}{\ind{2}, \ind{3}, \ind{5}, 1}\,
    \cpl{SSSS}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 1} \,\times\\
  & \frac{1}{2} \,\bigg\{
    \frac{1}{\epsilon}\, \m_{\ind{6}}^2\,
      \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2}
      - \tintm{1123}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/002.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSS}{\ind{2}, \ind{3}, \ind{5}, 1}\,
    \cpl{SSVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 1}\,\times\\
  & \bigg\{
    {-}\,\frac{2}{\epsilon}\, \m_{\ind{6}}^2\, \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2}
    + \left(2 - \deltaMS\,\epsilon\right)
      \tintm{1123}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/003.tex <==
$\begin{aligned}
  &\cpl{SSSS}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 1}\,\cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,\cpl{SSV}{\ind{2}, \ind{5}, \ind{3}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \,\Big[
      \aint{\m_{\ind{6}}^2}
      + \m_{\ind{6}}^2\, \yonesum{112}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2}
    \Big]\\
    &{-}\,\ysum{1123}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/004.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{3}, \ind{5}, 1}\,
    \cpl{SSVV}{\ind{6}, \ind{6}, \ind{4}, \ind{5}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \,\Big[
      {-}\, \aint{\m_{\ind{6}}^2}
       + \m_{\ind{6}}^2\,
         \yonesum{112}{[1]-2[2]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2}
    \Big]\\
    &{-}\,\ysum{1123}{[1]-2[2]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/005.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{5}, \ind{3}, 1}\,
    \cpl{SSVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 1}\,\times\\
  & \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon} \,\Big[
      2\,\m_{\ind{6}}^2\,
        \yonesum{112}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2}
      + \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{6}}^2}
    \Big]\\
    &{+} \left(2 - \deltaMS\,\epsilon\right)
      \ysum{1123}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/006.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{3}, \ind{5}, 1}\,\times\\
  & \!\Big[
    4\,\cpl{VVVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 1}
     + \cpl{VVVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 2}
     + \cpl{VVVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 3} \Big]\, \times\\
  & \frac{1}{4} \,\bigg\{
    \frac{1}{\epsilon} \,\Big[
      {-}\, 2\,\m_{\ind{6}}^2\,
        \yonesum{112}{[1]-2[2]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2}
      + \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{6}}^2}
    \Big]
  \!\bigg\}\\
  &{+}\,\cpl{SSV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
        \cpl{SSV}{\ind{2}, \ind{3}, \ind{5}, 1}\,\times\\
  & \!\Big[\!\left(4 - 2\,\deltaMS\,\epsilon\right)
      \cpl{VVVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 1}
    + \cpl{VVVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 2}
    + \cpl{VVVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 3} \Big]\, \times\\
  &\frac{1}{2} \,\bigg\{
    \ysum{1123}{[1]-2[2]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/007.tex <==
$\begin{aligned}
  & \cpl{SSVV}{\ind{6}, \ind{6}, \ind{4}, \ind{5}, 1}\,
    \cpl{SVV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{3}, \ind{5}, 1}\,\times\\
  & \begin{aligned}[t] \bigg\{
    &{-}\, \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
      \m_{\ind{6}}^2\,\toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2}\\
    &{+} \left(2 - \deltaMS\,\epsilon\right)
      \tintm{1123}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/008.tex <==
$\begin{aligned}
  & \cpl{SVV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{3}, \ind{5}, 1}\,\times\\
  & \!\Big[
    4\,\cpl{VVVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 1}
     + \cpl{VVVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 2}
     + \cpl{VVVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 3}
    \Big]\, \times\\
  & \bigg\{
    \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
      \m_{\ind{6}}^2\, \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2}
  \!\bigg\}\\
  & \cpl{SVV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{3}, \ind{5}, 1}\,\times\\
  & \!\Big[
    \!\left(4 - 2\,\deltaMS\,\epsilon\right)
      \cpl{VVVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 1}
    + \cpl{VVVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 2}
    + \cpl{VVVV}{\ind{4}, \ind{5}, \ind{6}, \ind{6}, 3}
    \Big]\, \times\\
  & \bigg\{
    {-} \left(2 - \deltaMS\,\epsilon\right)
      \tintm{1123}{\m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/009.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SSS}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SSSS}{\ind{2}, \ind{4}, \ind{5}, \ind{6}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{
    \frac{1}{\epsilon}\, \bint{p^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
    - \tintm{1234}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/010.tex <==
$\begin{aligned}
  & \cpl{SSSS}{\ind{2}, \ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{1}, \ind{6}, \ind{3}, 1}\,
    \cpl{SSV}{\ind{4}, \ind{5}, \ind{3}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    &\frac{1}{\epsilon} \,\Big[
      \aint{\m_{\ind{4}}^2} - \aint{\m_{\ind{5}}^2}
    \Big]\\
    &{+}\, \yint{1234}{5}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2}
      - \yint{1234}{5}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/011.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SSVV}{\ind{2}, \ind{6}, \ind{4}, \ind{5}, 1}\,
    \cpl{SVV}{\ind{3}, \ind{4}, \ind{5}, 1}\,\times\\
  & \bigg\{
    \frac{2}{\epsilon}\,\bint{p^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
    - \left(2 - \deltaMS\,\epsilon\right)
      \tintm{1234}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/012.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SSVV}{\ind{2}, \ind{4}, \ind{5}, \ind{6}, 1}\,\times\\
  & \frac{1}{4} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \,\Big[
      4\, \aint{\m_{\ind{4}}^2}
      + 3\,\yonesum{12}{3[1]-[2]+[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2}
      + 4 \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{5}}^2}
    \Big]\\
    &{-}\, 2\,\ysum{1234}{4[1]-[2]-[3]+2[4]-[5]+2[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/013.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{6}, \ind{3}, 1}\,
    \cpl{SSVV}{\ind{2}, \ind{6}, \ind{4}, \ind{5}, 1}\,
    \cpl{VVV}{\ind{3}, \ind{4}, \ind{5}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon}\,\frac{3}{2} \left(2 - \deltaMS\,\epsilon\right)
      \left[\aint{\m_{\ind{4}}^2} - \aint{\m_{\ind{5}}^2}\right]\\
    &{-} \left(3 - 2\,\deltaMS\,\epsilon\right)
    \Big[
      \yint{1234}{5}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2}
      - \yint{1234}{5}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2}
    \Big]
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/014.tex <==
$\begin{aligned}
  & \cpl{SSVV}{\ind{2}, \ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{4}, \ind{3}, \ind{5}, 1}\,\times\\
  & 2 \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
      \bint{p^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}\\
    &{+} \left(2 - \deltaMS\,\epsilon\right)
      \tintm{1234}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/015.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/016.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/017.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/018.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/019.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/020.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/021.tex <==
$\begin{aligned}
  & \m_{\ind{3}}\,\m_{\ind{4}}\,\m_{\ind{6}}\,\m_{\ind{7}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{5}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{4}, \ind{7}, \ind{2}, 1}\,
          \cpl{FFS}{\ind{6}, \ind{7}, \ind{5}, 1}}\,\times\\
  & \frac{1}{2} \,\bigg\{
    \tintm{12345}{\m_{\ind{7}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{3}}\,\m_{\ind{4}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{5}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{4}, \ind{7}, \ind{2}, 1}\,
          \cpl{FFS}{\ind{6}, \ind{7}, \ind{5}, 2}}\,\times\\
  & \frac{1}{2} \,\bigg\{
    \ysum{12345}{[2] - [3] + [5]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{3}}\,\m_{\ind{7}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{5}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{4}, \ind{7}, \ind{2}, 2}\,
          \cpl{FFS}{\ind{6}, \ind{7}, \ind{5}, 2}}\,\times\\
  & \frac{1}{2} \,\bigg\{
    \ysum{12345}{[1] - [3] + [5] - [6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{3}}\,\m_{\ind{6}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{5}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{4}, \ind{7}, \ind{2}, 2}\,
          \cpl{FFS}{\ind{6}, \ind{7}, \ind{5}, 1}}\,\times\\
  & \frac{1}{2} \,\bigg\{
    {-}\, \frac{2}{\epsilon}\,\bint{p^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
    + \ysum{12345}{[4] + [5] - [6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}\\
  &{+}\,\Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{5}, 1}\,
              \cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 2}\,
              \cpl{FFS}{\ind{4}, \ind{7}, \ind{2}, 2}\,
              \cpl{FFS}{\ind{6}, \ind{7}, \ind{5}, 1}}\,\times\\
  & \frac{1}{4} \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{2}{\epsilon} \,\Big[
      \aint{\m_{\ind{5}}^2}
      + \yonesum{12}{[1] + [2] - [6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2}
    \Big]\\
    &{+}\, \ysum{12345}{2[15]-[36]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+} \left[\left(\ind{3},\ind{4}\right)\leftrightarrow\left(\ind{6},\ind{7}\right)\right]
  + \left[\left(\ind{1},\ind{3},\ind{6}\right)\leftrightarrow\left(\ind{2},\ind{4},\ind{7}\right)\right]
  + \left[\left(\ind{1},\ind{3},\ind{4}\right)\leftrightarrow\left(\ind{2},\ind{7},\ind{6}\right)\right]
\end{aligned}$


==> TeX/Selfs/022.tex <==
$\begin{aligned}
  & \m_{\ind{3}}\,\m_{\ind{5}}\,\m_{\ind{6}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{5}, \ind{4}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{5}, \ind{6}, \ind{7}, 1}}\,
          \cpl{SSS}{\ind{2}, \ind{4}, \ind{7}, 1}\,\times\\
  & \bigg\{
  \tintm{12345}{\m_{\ind{7}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{3}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{5}, \ind{4}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{5}, \ind{6}, \ind{7}, 2}}\,
          \cpl{SSS}{\ind{2}, \ind{4}, \ind{7}, 1}\,\times\\
  & \bigg\{
    {-}\, \frac{2}{\epsilon} \,\bint{p^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
     + \ysum{12345}{[2] + [3] - [5]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{5}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{5}, \ind{4}, 1}\,
      \cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 2}\,
      \cpl{FFS}{\ind{5}, \ind{6}, \ind{7}, 1}}\,
      \cpl{SSS}{\ind{2}, \ind{4}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{
    {-}\, \frac{2}{\epsilon} \,\bint{p^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
     + \ysum{12345}{2[1]-[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}\\
  &{+} \left[\left(\ind{3},\ind{4}\right)\leftrightarrow\left(\ind{6},\ind{7}\right)\right]
\end{aligned}$


==> TeX/Selfs/023.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/024.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SSS}{\ind{2}, \ind{4}, \ind{7}, 1}\,
    \cpl{SSS}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SSS}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{
    {-}\,\tintm{12345}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/025.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SUU}{\ind{2}, -\ind{7}, \ind{4}, 1}\,
    \cpl{SUU}{\ind{3}, -\ind{4}, \ind{5}, 1}\,
    \cpl{SUU}{\ind{6}, -\ind{5}, \ind{7}, 1}\,\times\\
  & \frac{1}{2}\,\bigg\{
    \tintm{12345}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/026.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/027.tex <==
$\begin{aligned}
  & \cpl{SUU}{\ind{1}, -\ind{3}, \ind{6}, 1}\,
    \cpl{SUU}{\ind{2}, -\ind{7}, \ind{4}, 1}\,
    \cpl{SUU}{\ind{5}, -\ind{4}, \ind{3}, 1}\,
    \cpl{SUU}{\ind{5}, -\ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{
    \tintm{12345}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/028.tex <==
$\begin{aligned}
  & \m_{\ind{3}}\,\m_{\ind{4}}\,\m_{\ind{6}}\,\m_{\ind{7}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{4}, \ind{7}, \ind{2}, 2}\,
          \cpl{FFV}{\ind{3}, \ind{4}, \ind{5}, 2}\,
          \cpl{FFV}{\ind{6}, \ind{7}, \ind{5}, 2}}\,\times\\
  & \bigg\{
    \!\!\left(2 - \deltaMS\,\epsilon\right)
    \tintm{12345}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{3}}\,\m_{\ind{4}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{4}, \ind{7}, \ind{2}, 2}\,
          \cpl{FFV}{\ind{3}, \ind{4}, \ind{5}, 2}\,
          \cpl{FFV}{\ind{6}, \ind{7}, \ind{5}, 1}}\,\times\\
  & \bigg\{
    {-} \left(1 - \deltaMS\,\epsilon\right)
      \ysum{12345}{[2]-[3]+[5]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{3}}\,\m_{\ind{7}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{4}, \ind{7}, \ind{2}, 1}\,
          \cpl{FFV}{\ind{3}, \ind{4}, \ind{5}, 2}\,
          \cpl{FFV}{\ind{6}, \ind{7}, \ind{5}, 1}}\,\times\\
  & \bigg\{
    {-} \left(1 - \deltaMS\,\epsilon\right)
      \ysum{12345}{[1]-[3]+[5]-[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{3}}\,\m_{\ind{6}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{4}, \ind{7}, \ind{2}, 1}\,
          \cpl{FFV}{\ind{3}, \ind{4}, \ind{5}, 2}\,
          \cpl{FFV}{\ind{6}, \ind{7}, \ind{5}, 2}}\,\times\\
  & \bigg\{
    {-}\, \frac{4}{\epsilon}\, \bint{p^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
    + \left(2 - \deltaMS\,\epsilon\right)
    \ysum{12345}{[4]+[5]-[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}\\
  &{+}\,\Real{\cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
              \cpl{FFS}{\ind{4}, \ind{7}, \ind{2}, 2}\,
              \cpl{FFV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
              \cpl{FFV}{\ind{6}, \ind{7}, \ind{5}, 1}}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{2}{\epsilon} \,\Big[
      2\,\yonesum{12}{[1]+[2]-[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2}
      + \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{5}}^2}
    \Big]\\
    &{+}\, \ysum{12345}{2[14]-4[16]+[36]+[66]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}\\
    &{+} \left(1 - \deltaMS\,\epsilon\right)
       \ysum{12345}{2[15]-[36]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+} \left[\left(\ind{3},\ind{4}\right)\leftrightarrow\left(\ind{6},\ind{7}\right)\right]
  + \left[\left(\ind{1},\ind{3},\ind{6}\right)\leftrightarrow\left(\ind{2},\ind{4},\ind{7}\right)\right]
  + \left[\left(\ind{1},\ind{3},\ind{4}\right)\leftrightarrow\left(\ind{2},\ind{7},\ind{6}\right)\right]  
\end{aligned}$


==> TeX/Selfs/029.tex <==
$\begin{aligned}
  & \m_{\ind{3}}\,\m_{\ind{5}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{5}, \ind{4}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFV}{\ind{5}, \ind{6}, \ind{7}, 2}}\,
          \cpl{SSV}{\ind{2}, \ind{4}, \ind{7}, 1}\,\times\\
  & 2 \,\bigg\{
    {-}\,\ysum{12345}{2[1]-[2]-[3]+[5]-2[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}\\
  &{+}\,\m_{\ind{3}}\,\m_{\ind{6}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{5}, \ind{4}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 2}\,
          \cpl{FFV}{\ind{5}, \ind{6}, \ind{7}, 1}}\,
          \cpl{SSV}{\ind{2}, \ind{4}, \ind{7}, 1}\,\times\\
  & 2 \,\bigg\{
    {-}\, \frac{2}{\epsilon}\,\bint{p^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
    - \ysum{12345}{2[1]-[2]-[3]-2[4]+[5]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{5}}\,\m_{\ind{6}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{5}, \ind{4}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 2}\,
          \cpl{FFV}{\ind{5}, \ind{6}, \ind{7}, 2}}\,
          \cpl{SSV}{\ind{2}, \ind{4}, \ind{7}, 1}\,\times\\
  & 2 \,\bigg\{
    {-}\,\ysum{12345}{2[1]-[2]-[3]+[4]+[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}\\
  &{+}\,\Real{\cpl{FFS}{\ind{3}, \ind{5}, \ind{4}, 1}\,
              \cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
              \cpl{FFV}{\ind{5}, \ind{6}, \ind{7}, 1}}\,
              \cpl{SSV}{\ind{2}, \ind{4}, \ind{7}, 1}\,\times\\
  & 2 \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \,\Big[
      {-}\,\yonesum{12}{[1]+[2]-[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2}
       - \yonesum{12}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2}
      \Big]\\
      &{-}\, \ysum{12345}{2[11]-[12]-[13]-2[14]-[24]+2[15]-2[16]-[36]+2[46]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/030.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/031.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SSS}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{4}, \ind{7}, 1}\,
    \cpl{SSV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \bigg\{
    {-}\, \frac{1}{\epsilon}\,\bint{p^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
    - \ysum{12345}{2[1]-[2]-[3]-[4]+[5]-[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/032.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/033.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SSS}{\ind{2}, \ind{4}, \ind{7}, 1}\,
    \cpl{SSV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SSV}{\ind{6}, \ind{7}, \ind{5}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \,\Big[
      \bint{p^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2} + \bint{p^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \Big]\\
    &{-}\, \ysum{12345}{[1]+[2]-[3]+[4]+[5]-2[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/034.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SUU}{\ind{2}, -\ind{7}, \ind{4}, 1}\,
    \cpl{SUU}{\ind{3}, -\ind{4}, \ind{5}, 1}\,
    \cpl{UUV}{-\ind{5}, \ind{7}, \ind{6}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{
    \frac{2}{\epsilon}\,\bint{p^2, \m_{\ind{7}}^2, \m_{\ind{4}}^2}
    - \ysum{12345}{2[1]-[2]+[3]-2[4]+[5]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}\\
  &{+}\,\cpl{SSV}{\ind{1}, \ind{3}, \ind{6}, 1}\,
        \cpl{SUU}{\ind{2}, \ind{7}, -\ind{4}, 1}\,
        \cpl{SUU}{\ind{3}, \ind{4}, -\ind{5}, 1}\,
        \cpl{UUV}{\ind{5}, -\ind{7}, \ind{6}, 2}\,\times\\
  & \frac{1}{2} \,\bigg\{
    {-}\, \ysum{12345}{[2]-[3]+2[4]-[5]-2[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/035.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/036.tex <==
$\begin{aligned}
  & \cpl{SUU}{\ind{1}, -\ind{3}, \ind{6}, 1}\,
    \cpl{SUU}{\ind{2}, -\ind{7}, \ind{4}, 1}\,
    \cpl{UUV}{-\ind{4}, \ind{3}, \ind{5}, 1}\,
    \cpl{UUV}{-\ind{6}, \ind{7}, \ind{5}, 1}\,\times\\
&  \frac{1}{2}  \,\bigg\{ %% added factor of 2
    {-}\,\ysum{12345}{[1]-[3]+[5]-[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}
%  &{+} \left[\left(\ind{3},\ind{4}\right)\leftrightarrow\left(\ind{6},\ind{7}\right)\right]
\end{aligned}$
% $\begin{aligned}
%   & \cpl{SUU}{\ind{1}, -\ind{3}, \ind{6}, 1}\,
%     \cpl{SUU}{\ind{2}, -\ind{7}, \ind{4}, 1}\,
%     \cpl{UUV}{-\ind{4}, \ind{3}, \ind{5}, 1}\,
%     \cpl{UUV}{-\ind{6}, \ind{7}, \ind{5}, 1}\,\times\\
% &  \frac{1}{4}  \,\bigg\{ 
%     {-}\,\ysum{12345}{[1]-[3]+[5]-[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
%   \!\bigg\} \\
% & + \cpl{SUU}{\ind{1}, \ind{3}, -\ind{6}, 1}\,
%     \cpl{SUU}{\ind{2}, \ind{7}, -\ind{4}, 1}\,
%     \cpl{UUV}{\ind{4}, -\ind{3}, \ind{5}, 2}\,
%     \cpl{UUV}{\ind{6}, -\ind{7}, \ind{5}, 2}\,\times\\
% &  \frac{1}{4}  \,\bigg\{ 
%     {-}\,\ysum{12345}{[1]-[3]+[5]-[6]}{\m_{\ind{6}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{7}}^2, \m_{\ind{4}}^2} \!\bigg\}\\
% &{\color{red} Mark EDITED}
% %  &{+} \left[\left(\ind{3},\ind{4}\right)\leftrightarrow\left(\ind{6},\ind{7}\right)\right]
% \end{aligned}$


==> TeX/Selfs/037.tex <==
$\begin{aligned}
  & \m_{\ind{3}}\,\m_{\ind{5}}\,\m_{\ind{6}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFV}{\ind{3}, \ind{5}, \ind{4}, 2}\,
          \cpl{FFV}{\ind{5}, \ind{6}, \ind{7}, 1}}\,
          \cpl{SVV}{\ind{2}, \ind{4}, \ind{7}, 1}\,\times\\
  & 2 \,\bigg\{
    \!\!\left(2 - \deltaMS\,\epsilon\right)
    \tintm{12345}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}\\
  &{+}\,\m_{\ind{3}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFV}{\ind{3}, \ind{5}, \ind{4}, 2}\,
          \cpl{FFV}{\ind{5}, \ind{6}, \ind{7}, 2}}\,
          \cpl{SVV}{\ind{2}, \ind{4}, \ind{7}, 1}\,\times\\
  & 2 \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
      \bint{p^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}\\
    &{-} \left(1 - \deltaMS\,\epsilon\right)
      \ysum{12345}{[2]+[3]-[5]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+}\,\m_{\ind{5}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{6}, \ind{1}, 1}\,
          \cpl{FFV}{\ind{3}, \ind{5}, \ind{4}, 1}\,
          \cpl{FFV}{\ind{5}, \ind{6}, \ind{7}, 2}}\,
          \cpl{SVV}{\ind{2}, \ind{4}, \ind{7}, 1}\,\times\\
  & \begin{aligned}[t] \bigg\{
    &{-}\, \frac{2}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
      \bint{p^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}\\
    &{+} \left(2 - \deltaMS\,\epsilon\right)
      \ysum{12345}{[1]+[2]-[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+} \left[\left(\ind{3},\ind{4}\right)\leftrightarrow\left(\ind{6},\ind{7}\right)\right]  
\end{aligned}$


==> TeX/Selfs/038.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/039.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SSV}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{4}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{
    \ysum{12345}{2[1]-[2]-[3]+2[4]-[5]+4[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/040.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{3}, \ind{5}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{5}, \ind{6}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{4}, \ind{7}, 1}\,\times\\
  & \frac{1}{4} \begin{aligned}[t] \,\bigg\{
    & \frac{2}{\epsilon} \,\Big[
      \bint{p^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
      + 2 \left(2 - \deltaMS\,\epsilon\right) \bint{p^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \Big]\\
    &{-}\, \ysum{12345}{2[1]+2[2]+4[3]-[4]-[5]-[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/041.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{7}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{3}, \ind{5}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{5}, \ind{7}, \ind{6}, 1}\,\times\\
  & \begin{aligned}[t] \bigg\{
    & \frac{1}{\epsilon} \,\Big[
      - \aint{\m_{\ind{5}}^2}
      - \yonesum{12}{2[1]-[2]+2[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2}
      + \yonesum{12}{[1]-2[2]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \Big]\\
    &{+}\, \ysum{12345}{\left([1]-[2]+[3]-2[4]+[5]+[6]\right)
                        \left([1]-2[2]+[3]-[4]+[5]+[6]\right)}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/042.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/043.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{4}, \ind{7}, 1}\,
    \cpl{SSV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SVV}{\ind{6}, \ind{5}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{
    {-}\, \frac{2}{\epsilon}\, \bint{p^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2}
    + \ysum{12345}{2[1]-[2]-[3]+4[4]-[5]+2[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/044.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/045.tex <==
% $\begin{aligned}
%   & \cpl{SUU}{\ind{1}, -\ind{6}, \ind{3}, 1}\,
%     \cpl{SVV}{\ind{2}, \ind{4}, \ind{7}, 1}\,
%     \cpl{UUV}{-\ind{3}, \ind{5}, \ind{4}, 1}\,
%     \cpl{UUV}{-\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
%   & \frac{1}{4} \begin{aligned}[t] \,\bigg\{
%     &{-}\, \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
%       \bint{p^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}\\
%     &{+}\,\ysum{12345}{[1]+[3]-[4]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
%     \!\bigg\}
%   \end{aligned}\\
%   &{+} \left[\left(\ind{3},\ind{4}\right)\leftrightarrow\left(\ind{6},\ind{7}\right)\right]
% \end{aligned}$
$\begin{aligned}
  & \cpl{SUU}{\ind{1}, -\ind{6}, \ind{3}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{4}, \ind{7}, 1}\,
    \cpl{UUV}{-\ind{3}, \ind{5}, \ind{4}, 1}\,
    \cpl{UUV}{-\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{%% added factor of 2
    &{-}\, \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
      \bint{p^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}\\
    &{+}\,\ysum{12345}{[1]+[3]-[4]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}
  \end{aligned}
%  &{+} \left[\left(\ind{3},\ind{4}\right)\leftrightarrow\left(\ind{6},\ind{7}\right)\right]
\end{aligned}$


==> TeX/Selfs/046.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/047.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{3}, \ind{5}, \ind{4}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{4}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{2}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
      \bint{p^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}\\
    &{+}\,\ysum{12345}{5[1]-2[2]+[3]-2[4]+[5]+[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/048.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/049.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{4}, \ind{7}, 1}\,
    \cpl{SSV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{VVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{3}{\epsilon}\,
      \yonesum{12}{2[1]-[2]+2[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2}\\
    &{+}\, 2\,\ysum{12345}{2[11]-2[12]-2[13]-[14]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}\\
    &{+}\, \frac{1}{2}\,\ysum{12345}{2[22]+4[23]+[33]+2[25]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}\\
    &{-}\, 2\,\ysum{12345}{2[16]+2[26]-[66]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+} \left[\left(\ind{1},\ind{3},\ind{6}\right)\leftrightarrow\left(\ind{2},\ind{4},\ind{7}\right)\right]
\end{aligned}$


==> TeX/Selfs/050.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{4}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SVV}{\ind{6}, \ind{5}, \ind{7}, 1}\,\times\\
  & \bigg\{
    \!\!\left(2 - \deltaMS\,\epsilon\right)
    \tintm{12345}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/051.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{7}, \ind{4}, 1}\,
    \cpl{SVV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SVV}{\ind{7}, \ind{5}, \ind{6}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{
    \ysum{12345}{[1]-2[2]+[3]-2[4]+[5]+5[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/052.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/053.tex <==
$\begin{aligned}
  & \cpl{SVV}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{4}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{5}, \ind{3}, \ind{4}, 1}\,
    \cpl{SVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \bigg\{
    {-} \left(2 - \deltaMS\,\epsilon\right)
      \tintm{12345}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/054.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{4}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{VVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{3}{\epsilon} \left(2 - \deltaMS\,\,\epsilon\right)
      \bint{p^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}\\
    &{-}\, 2 \left(3 - 2\, \deltaMS\,\,\epsilon\right)
      \ysum{12345}{[1]-[2]+[3]-2[4]+[5]+[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/055.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/056.tex <==
$\begin{aligned}
  & \cpl{SVV}{\ind{1}, \ind{3}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{4}, \ind{7}, 1}\,
    \cpl{VVV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{VVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{3}{4} \begin{aligned}[t] \,\bigg\{
    & \frac{6}{\epsilon} \left(2 - \deltaMS\,\epsilon\right) \left[
      \bint{p^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2} + \bint{p^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
      \right]\\
    &{-} \left(3 - 2\, \deltaMS\,\epsilon\right)
      \ysum{12345}{[1]+[2]+2[3]+[4]+[5]-2[6]}{\m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2, \m_{\ind{4}}^2, \m_{\ind{7}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/057.tex <==
$\begin{aligned}
  & \m_{\ind{3}}\,\m_{\ind{4}}\,\m_{\ind{5}}\,\m_{\ind{7}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{7}, \ind{2}, 1}\,
          \cpl{FFS}{\ind{4}, \ind{5}, \ind{6}, 1}\,
          \cpl{FFS}{\ind{5}, \ind{7}, \ind{6}, 1}}\,\times\\
  & 2 \,\bigg\{
    {-}\, \frac{1}{\epsilon}\,
      \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    + \tintm{11234}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{3}}\,\m_{\ind{5}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{7}, \ind{2}, 1}\,
          \cpl{FFS}{\ind{4}, \ind{5}, \ind{6}, 2}\,
          \cpl{FFS}{\ind{5}, \ind{7}, \ind{6}, 2}}\,\times\\
  & 2 \,\bigg\{
    {-}\, \frac{1}{\epsilon}\,
      \yoneint{112}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
     + \yint{11234}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{4}}\,\m_{\ind{7}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{7}, \ind{2}, 2}\,
          \cpl{FFS}{\ind{4}, \ind{5}, \ind{6}, 1}\,
          \cpl{FFS}{\ind{5}, \ind{7}, \ind{6}, 2}}\,\times\\
  & \frac{1}{2} \,\bigg\{
    {-}\, \frac{1}{\epsilon}\,
      \yonesum{112}{[1]+[2]-[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    + 2\,\ysum{11234}{[2]+[3]-[5]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{3}}\,\m_{\ind{4}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{7}, \ind{2}, 1}\,
          \cpl{FFS}{\ind{4}, \ind{5}, \ind{6}, 1}\,
          \cpl{FFS}{\ind{5}, \ind{7}, \ind{6}, 2}}\,\times\\
  & 2 \,\bigg\{
    {-}\, \frac{1}{\epsilon}\,
      \yoneint{112}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    + \ysum{11234}{[1]+[3]-[4]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{4}}\,\m_{\ind{5}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{7}, \ind{2}, 2}\,
          \cpl{FFS}{\ind{4}, \ind{5}, \ind{6}, 1}\,
          \cpl{FFS}{\ind{5}, \ind{7}, \ind{6}, 1}}\,\times\\
  & 2 \,\bigg\{
    {-}\, \frac{1}{\epsilon}\,
      \yonesum{112}{[1]+[2]-[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    + \ysum{11234}{[1]+[2]-[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}\\
  &{+}\,\Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{1}, 1}\,
              \cpl{FFS}{\ind{3}, \ind{7}, \ind{2}, 2}\,
              \cpl{FFS}{\ind{4}, \ind{5}, \ind{6}, 2}\,
              \cpl{FFS}{\ind{5}, \ind{7}, \ind{6}, 1}}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon} \,\Big[
      4\,\aint{\m_{\ind{6}}^2}
      + \yonesum{112}{[11]+[12]-[16]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
      \Big]\\
    &{+}\, 2\,\ysum{11234}{[12]+[14]-[15]-[23]+[36]+[24]-[46]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+} \left[\left(\ind{1},\ind{4}\right)\leftrightarrow\left(\ind{2},\ind{7}\right)\right]
\end{aligned}$


==> TeX/Selfs/058.tex <==
$\begin{aligned}
  & \m_{\ind{5}}\,\m_{\ind{6}}\,
    \Real{\cpl{FFS}{\ind{5}, \ind{6}, \ind{4}, 1}\,
          \cpl{FFS}{\ind{5}, \ind{6}, \ind{7}, 1}}\,
          \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
          \cpl{SSS}{\ind{2}, \ind{3}, \ind{7}, 1}\,\times\\
  & 2\,\bigg\{
    {-}\, \frac{1}{\epsilon}\,
      \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    + \tintm{11234}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}\\
  &{+}\,\Real{\cpl{FFS}{\ind{5}, \ind{6}, \ind{4}, 1}\,
              \cpl{FFS}{\ind{5}, \ind{6}, \ind{7}, 2}}\,
              \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
              \cpl{SSS}{\ind{2}, \ind{3}, \ind{7}, 1}\,\times\\
  & \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \,\Big[
      {-}\,2 \left(\m_{\ind{5}}^2 + \m_{\ind{6}}^2\right)
        \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
       + \yoneint{112}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    \Big]\\
    &{-}\, \ysum{11234}{[1]-[3]-[4]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/059.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSS}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{SSS}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{SSS}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{
    \frac{1}{\epsilon}\,\toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    - \tintm{11234}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/060.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSS}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{SUU}{\ind{4}, -\ind{5}, \ind{6}, 1}\,
    \cpl{SUU}{\ind{7}, -\ind{6}, \ind{5}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{
    {-}\,\frac{1}{\epsilon}\,
      \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    + \tintm{11234}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/061.tex <==
$\begin{aligned}
  & \cpl{SUU}{\ind{1}, -\ind{3}, \ind{4}, 1}\,
    \cpl{SUU}{\ind{2}, -\ind{7}, \ind{3}, 1}\,
    \cpl{SUU}{\ind{5}, -\ind{4}, \ind{6}, 1}\,
    \cpl{SUU}{\ind{5}, -\ind{6}, \ind{7}, 1}\,\times\\
  & \bigg\{
    {-}\,\frac{1}{\epsilon}\,
      \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    + \tintm{11234}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/062.tex <==
$\begin{aligned}
  & \m_{\ind{3}}\,\m_{\ind{4}}\,\m_{\ind{5}}\,\m_{\ind{7}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{7}, \ind{2}, 1}\,
          \cpl{FFV}{\ind{4}, \ind{5}, \ind{6}, 2}\,
          \cpl{FFV}{\ind{5}, \ind{7}, \ind{6}, 1}}\,\times\\
  & 4 \,\bigg\{
    \frac{2}{\epsilon}\, \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    - \left(2 - \deltaMS\,\epsilon\right)
    \tintm{11234}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{3}}\,\m_{\ind{4}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{7}, \ind{2}, 1}\,
          \cpl{FFV}{\ind{4}, \ind{5}, \ind{6}, 2}\,
          \cpl{FFV}{\ind{5}, \ind{7}, \ind{6}, 2}}\,\times\\
  & 4 \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon}\,
       \yoneint{112}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
    &{+} \left(1 - \deltaMS\,\epsilon\right)
        \ysum{11234}{[1]+[3]-[4]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+}\,\m_{\ind{4}}\,\m_{\ind{5}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{7}, \ind{2}, 2}\,
          \cpl{FFV}{\ind{4}, \ind{5}, \ind{6}, 2}\,
          \cpl{FFV}{\ind{5}, \ind{7}, \ind{6}, 1}}\,\times\\
  & 4 \begin{aligned}[t] \,\bigg\{
    & \frac{2}{\epsilon}\,
      \yonesum{112}{[1]+[2]-[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
    &{-} \left(2 - \deltaMS\,\epsilon\right)
        \ysum{11234}{[1]+[2]-[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}
  \end{aligned}\\
  &{+}\,\m_{\ind{3}}\,\m_{\ind{5}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{7}, \ind{2}, 1}\,
          \cpl{FFV}{\ind{4}, \ind{5}, \ind{6}, 1}\,
          \cpl{FFV}{\ind{5}, \ind{7}, \ind{6}, 2}}\,\times\\
  & 4 \,\bigg\{
    \frac{2}{\epsilon}\, \yoneint{112}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    - \left(2 - \deltaMS\,\epsilon\right)
  \yint{11234}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}\\
  &{+}\,\m_{\ind{4}}\,\m_{\ind{7}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{7}, \ind{2}, 2}\,
          \cpl{FFV}{\ind{4}, \ind{5}, \ind{6}, 2}\,
          \cpl{FFV}{\ind{5}, \ind{7}, \ind{6}, 2}}\,\times\\
  & \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon}\,
      \yonesum{112}{[1]+[2]-[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
    &{+}\,2 \left(1 - \deltaMS\,\epsilon\right)
      \ysum{11234}{[2]+[3]-[5]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+}\,\Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{1}, 1}\,
              \cpl{FFS}{\ind{3}, \ind{7}, \ind{2}, 2}\,
              \cpl{FFV}{\ind{4}, \ind{5}, \ind{6}, 1}\,
              \cpl{FFV}{\ind{5}, \ind{7}, \ind{6}, 1}}\,\times\\
  & \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon} \,\Big[
      \yonesum{112}{[11]+[12]-[16]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
      + 2 \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{6}}^2}
    \Big]\\
    &{+}\, 2 \left(1 - \deltaMS\,\epsilon\right)
      \ysum{11234}{[12]+[13]-[15]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+} \left[\left(\ind{1},\ind{4}\right)\leftrightarrow\left(\ind{2},\ind{7}\right)\right]
\end{aligned}$


==> TeX/Selfs/063.tex <==
$\begin{aligned}
  & \m_{\ind{5}}\,\m_{\ind{6}}\,
    \Real{\cpl{FFS}{\ind{5}, \ind{6}, \ind{4}, 1}\,
          \cpl{FFS}{\ind{5}, \ind{6}, \ind{7}, 1}}\,
          \cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,
          \cpl{SSV}{\ind{2}, \ind{7}, \ind{3}, 1}\,\times\\
  & 2 \,\bigg\{
    {-}\, \frac{1}{\epsilon}\,
      \yonesum{112}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
     + \ysum{11234}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}\\
  &{+}\,\Real{\cpl{FFS}{\ind{5}, \ind{6}, \ind{4}, 1}\,
              \cpl{FFS}{\ind{5}, \ind{6}, \ind{7}, 2}}\,
              \cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,
              \cpl{SSV}{\ind{2}, \ind{7}, \ind{3}, 1}\,\times\\
  & \begin{aligned}[t] \bigg\{
    & \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      &\yonesum{112}{2[11]-[12]+2[16])}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
      &{-}\, 2 \left(\m_{\ind{5}}^2 + \m_{\ind{6}}^2\right)
        \yonesum{112}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
      \Big]
    \end{aligned}\\
    &{-}\, \ysum{11234}{([1]-[3]-[4])(2[1]-[2]+2[6])}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}  
\end{aligned}$


==> TeX/Selfs/064.tex <==
$\begin{aligned}
  & \m_{\ind{5}}\,
    \Real{\cpl{FFS}{\ind{5}, \ind{6}, \ind{4}, 1}\,
          \cpl{FFV}{\ind{5}, \ind{6}, \ind{7}, 2}}\,
          \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
          \cpl{SSV}{\ind{2}, \ind{3}, \ind{7}, 1}\,\times\\
  & \bigg\{
    \frac{1}{\epsilon}\,\yonesum{112}{[2]-[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    - \ysum{11234}{[1]-[3]-[4]+2[5]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}\\
  &{+} \left[\ind{5}\leftrightarrow\ind{6}\right]
\end{aligned}$


==> TeX/Selfs/065.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/066.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{SSS}{\ind{5}, \ind{6}, \ind{7}, 1}\,
    \cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{7}, \ind{3}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \,\Big[
      \yonesum{112}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
      \Big]\\
    &{-}\, \ysum{11234}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/067.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSS}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{SSV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{
    \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2}
    - \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/068.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/069.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSS}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{SSV}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{5}, \ind{7}, \ind{6}, 1}\,\times\\
  & \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon} \,\Big[
      \left(\m_{\ind{5}}^2 + \m_{\ind{6}}^2\right)
        \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
      - 2\,\yoneint{112}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    \Big]\\
    &{+}\,\ysum{11234}{2[1]+2[3]-[4]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/070.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{7}, \ind{3}, 1}\,
    \cpl{SUU}{\ind{4}, -\ind{5}, \ind{6}, 1}\,
    \cpl{SUU}{\ind{7}, -\ind{6}, \ind{5}, 1}\,\times\\
  &\frac{1}{2} \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon}\,
      \yonesum{112}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
    &{+}\,\ysum{11234}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/071.tex <==
% $\begin{aligned}
%   & \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
%     \cpl{SSV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
%     \cpl{SUU}{\ind{4}, -\ind{5}, \ind{6}, 1}\,
%     \cpl{UUV}{-\ind{6}, \ind{5}, \ind{7}, 1}\,\times\\
%   & \frac{1}{4} \begin{aligned}[t] \,\bigg\{
%     & \frac{1}{\epsilon}\,
%       \yonesum{112}{[2]-[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
%     - \ysum{11234}{[2]-[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
%     &{+}\, \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2}
%     - \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
%     \!\bigg\}
%   \end{aligned}\\
%   &{+} \left[\ind{5}\leftrightarrow\ind{6}\right]
% \end{aligned}$
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{SUU}{\ind{4}, -\ind{5}, \ind{6}, 1}\,
    \cpl{UUV}{-\ind{6}, \ind{5}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{%% added factor of 2
    & \frac{1}{\epsilon}\,
      \yonesum{112}{[2]-[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    - \ysum{11234}{[2]-[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
    &{+}\, \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2}
    - \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
 % &{+} \left[\ind{5}\leftrightarrow\ind{6}\right]
\end{aligned}$


==> TeX/Selfs/072.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/073.tex <==
$\begin{aligned}
  & \begin{aligned}[t] \!\Big[
    & \cpl{SUU}{\ind{1}, -\ind{3}, \ind{4}, 1}\,
      \cpl{SUU}{\ind{2}, -\ind{7}, \ind{3}, 1}\,
      \cpl{UUV}{-\ind{4}, \ind{5}, \ind{6}, 1}\,
      \cpl{UUV}{-\ind{5}, \ind{7}, \ind{6}, 1}\\
    &{+}\,\cpl{SUU}{\ind{1}, \ind{3}, -\ind{4}, 1}\,
          \cpl{SUU}{\ind{2}, \ind{7}, -\ind{3}, 1}\,
          \cpl{UUV}{\ind{4}, -\ind{5}, \ind{6}, 2}\,
          \cpl{UUV}{\ind{5}, -\ind{7}, \ind{6}, 2}
    \Big]\,\times
  \end{aligned}\\
  & \frac{1}{2} \,\bigg\{
    \frac{1}{\epsilon}\,
      \yoneint{112}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
      - \ysum{11234}{[1]+[3]-[4]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/074.tex <==
$\begin{aligned}
  & \m_{\ind{5}}\,
    \Real{\cpl{FFS}{\ind{5}, \ind{6}, \ind{4}, 1}\,
          \cpl{FFV}{\ind{5}, \ind{6}, \ind{7}, 2}}\,
          \cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,
          \cpl{SVV}{\ind{2}, \ind{3}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon}\, \yonesum{112}{3[1]-[2]+[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
    &{+}\, \ysum{11234}{3[1]-[2]-3[3]+3[4]+[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
    &{+}\, \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2}
      - \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+} \left[\ind{5}\leftrightarrow\ind{6}\right]
\end{aligned}$


==> TeX/Selfs/075.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/076.tex <==
$\begin{aligned}
  & \m_{\ind{5}}\,\m_{\ind{6}}\,
    \Real{\cpl{FFV}{\ind{5}, \ind{6}, \ind{4}, 1}\,
          \cpl{FFV}{\ind{5}, \ind{6}, \ind{7}, 1}}\,
          \cpl{SSV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
          \cpl{SSV}{\ind{2}, \ind{3}, \ind{7}, 1}\,\times\\
  & \bigg\{
    \frac{1}{\epsilon}\,\yonesum{112}{[1]-2[2]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    - \ysum{11234}{[1]-2[2]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}\\
  &{+}\,
    \Real{\cpl{FFV}{\ind{5}, \ind{6}, \ind{4}, 1}\,
          \cpl{FFV}{\ind{5}, \ind{6}, \ind{7}, 2}}\,
          \cpl{SSV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
          \cpl{SSV}{\ind{2}, \ind{3}, \ind{7}, 1}\,\times\\
  & \begin{aligned}[t] \bigg\{
    &{-}\, \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      & \m_{\ind{5}}^2\,\yonesum{112}{[1]-2[2]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
      &{+}\, \tfrac{1}{3}\,\yonesum{112}{([1]-[2]-[6])([1]-[2]-[6])-4[26]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
      \Big]
    \end{aligned}\\
    &{-}\, \ysum{11234}{[13]-[33]-[34]-2[26]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
    &{+}\, 2\, \ysum{11234}{[15]-[25]-[35]-[45]+[55]-[56]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+} \left[\ind{5}\leftrightarrow\ind{6}\right]
\end{aligned}$


==> TeX/Selfs/077.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,
    \cpl{SSV}{\ind{5}, \ind{6}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{3}, \ind{7}, 1}\,\times\\
  & \frac{1}{4} \begin{aligned}[t] \,\bigg\{
    & \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2}
    - \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
    &{-}\,3\,\ysum{11234}{[3]-[4]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/078.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/079.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{SSV}{\ind{5}, \ind{6}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      & \tfrac{1}{6}\,\yonesum{112}{([1]-[2]-[6])([1]-[2]-[6])-4[26]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
      &{-}\, \m_{\ind{5}}^2\,
        \yonesum{112}{[1]-2[2]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
        + \aint{\m_{\ind{5}}^2}
      \Big]
    \end{aligned}\\
    &{-}\, \ysum{11234}{[15]-[25]-[35]-[45]+2[55]-[56]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \bigg\}
  \end{aligned}\\
  &{+} \left[\ind{5}\leftrightarrow\ind{6}\right]
\end{aligned}$


==> TeX/Selfs/080.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{7}, \ind{3}, 1}\,
    \cpl{SSV}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{5}, \ind{7}, \ind{6}, 1}\,\times\\
  & \begin{aligned}[t] \bigg\{
    &{-}\, \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      & 2\,\yonesum{112}{2[11]-[12]+2[16]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
      &{+} \left(\m_{\ind{5}}^2 + \m_{\ind{6}}^2\right)
       \yonesum{112}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
      &{+}\, \aint{\m_{\ind{5}}^2}
        + 2 \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{6}}^2}
      \Big]
    \end{aligned}\\
    &{+}\, \ysum{11234}{\left(2[1]+2[3]-[4]\right)\left(2[1]-[2]+2[6]\right)}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/081.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{SSV}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{3}{\epsilon}\,
      \yonesum{112}{[2]-[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}}\\
    &{+}\, \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
      - \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2}\\
    &{-}\, 3\,\ysum{11234}{[2]-[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/082.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/083.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSS}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{7}, \ind{5}, \ind{6}, 1}\,\times\\
  & \bigg\{
    \frac{2}{\epsilon}\, \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    - \left(2 - \deltaMS\,\epsilon\right)
      \tintm{11234}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/084.tex <==
% $\begin{aligned}
%   & \cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,
%     \cpl{SUU}{\ind{4}, -\ind{5}, \ind{6}, 1}\,
%     \cpl{SVV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
%     \cpl{UUV}{-\ind{6}, \ind{5}, \ind{7}, 1}\,\times\\
%   & \frac{1}{8} \begin{aligned}[t] \,\bigg\{
%     &{-}\, \frac{1}{\epsilon}\,
%       \yonesum{112}{3[1]-[2]+[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
%     &{+}\, \ysum{11234}{3[1]-[2]-3[3]+3[4]+[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
%     &{+}\, \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2}
%       - \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
%     \!\bigg\}
%   \end{aligned}\\
%   &{+} \left[\ind{5}\leftrightarrow\ind{6}\right]
% \end{aligned}$
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,
    \cpl{SUU}{\ind{4}, -\ind{5}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{UUV}{-\ind{6}, \ind{5}, \ind{7}, 1}\,\times\\
  & \frac{1}{4} \begin{aligned}[t] \,\bigg\{ %%% added factor of 2
    &{-}\, \frac{1}{\epsilon}\,
      \yonesum{112}{3[1]-[2]+[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
    &{+}\, \ysum{11234}{3[1]-[2]-3[3]+3[4]+[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
    &{+}\, \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2}
      - \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
%  &{+} \left[\ind{5}\leftrightarrow\ind{6}\right]
\end{aligned}$


==> TeX/Selfs/085.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/086.tex <==
$\begin{aligned}
  & \begin{aligned}[t] \!\Big[
    & \cpl{SSV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
      \cpl{SSV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
      \cpl{UUV}{-\ind{5}, \ind{6}, \ind{4}, 1}\,
      \cpl{UUV}{-\ind{6}, \ind{5}, \ind{7}, 1}\\
    &{+}\,\cpl{SSV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
          \cpl{SSV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
          \cpl{UUV}{\ind{5}, -\ind{6}, \ind{4}, 2}\,
          \cpl{UUV}{\ind{6}, -\ind{5}, \ind{7}, 2}
    \Big]\,\times
  \end{aligned}\\
  & \frac{1}{8} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      &{-} \left(\m_{\ind{5}}^2 + \m_{\ind{6}}^2\right)
        \yonesum{112}{[1]-2[2]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
      &{+}\,\tfrac{1}{3}\,\yonesum{112}{([1]-2[2])([1]-2[6])-2[22]-2[66]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
      \Big]
    \end{aligned}\\
    &{-}\, 4\,\ysum{11234}{[15]-[25]-[35]-[45]+[55]-[56]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
    &{-}\, \ysum{11234}{\left([1]-2[2]-[3]-[4]\right)\left([1]-[3]-[4]-2[6]\right)}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/087.tex <==
$\begin{aligned}
  & \m_{\ind{5}}\,\m_{\ind{6}}\,
    \Real{\cpl{FFV}{\ind{5}, \ind{6}, \ind{4}, 1}\,
          \cpl{FFV}{\ind{5}, \ind{6}, \ind{7}, 1}}\,
          \cpl{SVV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
          \cpl{SVV}{\ind{2}, \ind{3}, \ind{7}, 1}\,\times\\
  & 2 \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
      \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
    &{+} \left(2 - \deltaMS\,\epsilon\right)
      \tintm{11234}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+}\,
    \Real{\cpl{FFV}{\ind{5}, \ind{6}, \ind{4}, 1}\,
          \cpl{FFV}{\ind{5}, \ind{6}, \ind{7}, 2}}\,
          \cpl{SVV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
          \cpl{SVV}{\ind{2}, \ind{3}, \ind{7}, 1}\,\times\\
  & \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      & 2 \left(2 - \deltaMS\,\epsilon\right)
        \m_{\ind{5}}^2\,\toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
      &{-}\, \tfrac{1}{3} \left(3 - 2\, \deltaMS\,\epsilon\right)
        \yoneint{112}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
      \Big]
    \end{aligned}\\
    &{+} \left(1 - \deltaMS\,\epsilon\right)
      \ysum{11234}{[1]-2[3]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+} \left[\ind{5}\leftrightarrow\ind{6}\right]
\end{aligned}$


==> TeX/Selfs/088.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{5}, \ind{6}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{5}, \ind{6}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{3}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      & 2 \left(2 - \deltaMS\,\epsilon\right)
        \left(\m_{\ind{5}}^2 + \m_{\ind{6}}^2\right)
        \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
      &{-}\, \tfrac{1}{3} \left(3 - 2\, \deltaMS\,\epsilon\right)
        \yoneint{112}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
      \!\Big]
    \end{aligned}\\
    &{+}\, \ysum{11234}{[1]-2[3]-2[4]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/089.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,
    \cpl{SSV}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{4} \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{3}{\epsilon} \,\Big[
      \yonesum{112}{3[1]-[2]+[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    \Big]\\
    &{+}\, \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
      - \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{6}}^2, \m_{\ind{5}}^2}\\
    &{+}\, 3\,\ysum{11234}{3[1]-[2]+[3]-[4]+[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/090.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/091.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{5}, \ind{4}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon}\,
      \yonesum{112}{[1]-2[2]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
    &{+}\, \ysum{11234}{[1]-2[2]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}  
\end{aligned}$


==> TeX/Selfs/092.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{7}, \ind{3}, 1}\,
    \cpl{SVV}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{7}, \ind{5}, \ind{6}, 1}\,\times\\
  & \begin{aligned}[t] \,\bigg\{
    & \frac{2}{\epsilon}\,
      \yonesum{112}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
    &{-} \left(2 - \deltaMS\,\epsilon\right)
      \ysum{11234}{2[1]-[2]+2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/093.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{VVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{
    \!\!\left(3 - 2\,\deltaMS\,\epsilon\right)
      \yint{11234}{5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}\\
  &{+} \left[\ind{5}\leftrightarrow\ind{6}\right]
\end{aligned}$


==> TeX/Selfs/094.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/095.tex <==
$\begin{aligned}
  & \begin{aligned} \!\Big[
    & \cpl{SVV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
      \cpl{SVV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
      \cpl{UUV}{-\ind{5}, \ind{6}, \ind{4}, 1}\,
      \cpl{UUV}{-\ind{6}, \ind{5}, \ind{7}, 1}\\
      &{+}\,\cpl{SVV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
            \cpl{SVV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
            \cpl{UUV}{\ind{5}, -\ind{6}, \ind{4}, 2}\,
            \cpl{UUV}{\ind{6}, -\ind{5}, \ind{7}, 2}
    \Big]\,\times
  \end{aligned}\\
  &\frac{1}{4} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      &{-}\,\tfrac{1}{3} \left(3 - \deltaMS\,\epsilon\right)
        \yoneint{112}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
      &{+} \left(2 - \deltaMS\,\epsilon\right)
        \left(\m_{\ind{5}}^2 + \m_{\ind{6}}^2\right)
        \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
    \Big]
    \end{aligned}\\
    &{+}\,\ysum{11234}{[1]-[3]-[4]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/096.tex <==
$\begin{aligned}
  & \cpl{SVV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{5}, \ind{4}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & 2 \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
      \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
    &{-} \left(2 - \deltaMS\,\epsilon\right)
    \tintm{11234}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/097.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{4}, \ind{3}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{SVV}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{VVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{4} \,\bigg\{
    \!\!\left(3 - 2\, \deltaMS\,\epsilon\right)
      \ysum{11234}{3[3]+5}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}\\
  &{+} \left[\ind{5}\leftrightarrow\ind{6}\right]
\end{aligned}$


==> TeX/Selfs/098.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/099.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{VVV}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{VVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{4} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      &{-}\, 3\, \yonesum{112}{\left([1]-[2]-[6]\right)\left([1]-[2]-[6]\right)-4[26]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
      &{-}\,\tfrac{1}{6}\,\yonesum{112}{[11]+4[22]+4[66]-2[12]-2[16]-8[26]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}\\
      &{-}\, 9\,\m_{\ind{5}}^2\,
        \yonesum{112}{[1]-2[2]-2[6]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
      + 3 \left(2 - \deltaMS\,\epsilon\right)\,\aint{\m_{\ind{5}}^2}
      \Big]
    \end{aligned}\\
    &{+} \left(3 - 2 \deltaMS\,\epsilon\right) \times\\
    &{\phantom{+}} \begin{aligned}[t] \Big[
      &{-}\, 6\,\ysum{11234}{\left([1]-[2]-[6]\right)\left([1]-[2]-[6]\right)-3[26]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
      &{-}\, 6\,\ysum{11234}{[15]-[25]-[35]-[45]+[55]-[56]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
      &{+}\, \tfrac{1}{2}\,\ysum{11234}{[11]-2[12]-2[16]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
      &{+}\, \ysum{11234}{4[13]-2[23]-3[33]-3[34]-2[36]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
      \Big]
    \end{aligned}\\
    &{+} \left(2 - \deltaMS\,\epsilon\right) \times\\
    &{\phantom{+}} \begin{aligned}[t] \Big[
      & 8\,\ysum{11234}{\left([1]-[2]-[6]\right)\left([1]-[2]-[6]\right)-4[26]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
      &{+}\, 4\,\ysum{11234}{[15]-[25]-[35]-[45]+[55]-[56]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
      &{+}\,\ysum{11234}{[11]-2[12]-2[16]+2[22]+2[66]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
      &{-}\, 2\,\ysum{11234}{2[23]-[33]-[34]+2[36]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
        \Big]
      \!\bigg\}
    \end{aligned}
  \end{aligned}\\
  &{+} \left[\ind{5}\leftrightarrow\ind{6}\right]
\end{aligned}$


==> TeX/Selfs/100.tex <==
$\begin{aligned}
  & \cpl{SVV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{3}, \ind{7}, 1}\,
    \cpl{VVV}{\ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{VVV}{\ind{5}, \ind{6}, \ind{7}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      & \!\left(2 - \deltaMS\,\epsilon\right) \left[
        9 \left(\m_{\ind{5}}^2 + \m_{\ind{6}}^2\right)
        \toneintm{112}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
        - \yoneint{112}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
        \right]\\
      &{+}\, \tfrac{11}{3} \left(3 - 2\, \deltaMS\,\epsilon\right)
        \yoneint{112}{1}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2}
      \Big]
    \end{aligned}\\
    &{-}\, 3 \left(3 - 2\, \deltaMS\,\epsilon\right)
      \ysum{11234}{[1]+[3]+[4]}{\m_{\ind{4}}^2, \m_{\ind{7}}^2, \m_{\ind{3}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/101.tex <==
$\begin{aligned}
  & \cpl{SSSS}{\ind{1}, \ind{2}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSSS}{\ind{3}, \ind{4}, \ind{5}, \ind{5}, 1}\,\times\\
  & \frac{1}{4} \,\bigg\{
    \frac{1}{\epsilon} \,\Big[
      \aint{\m_{\ind{5}}^2}
      + \m_{\ind{5}}^2\,\bint{0, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \Big]
    - \tintm{113}{\m_{\ind{3}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/102.tex <==
$\begin{aligned}
  & \cpl{SSSS}{\ind{1}, \ind{2}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSVV}{\ind{3}, \ind{4}, \ind{5}, \ind{5}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon} \,\Big[
      2\,\m_{\ind{5}}^2\,\bint{0, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
      + \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{5}}^2}
    \Big]\\
    &{+} \left(2 - \deltaMS\,\epsilon\right)
      \tintm{113}{\m_{\ind{3}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/103.tex <==
$\begin{aligned}
  & \cpl{SSVV}{\ind{1}, \ind{2}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSVV}{\ind{5}, \ind{5}, \ind{3}, \ind{4}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \,\Big[
      2\,\aint{\m_{\ind{5}}^2}
      + \left(2 - \deltaMS\,\epsilon\right)
      \m_{\ind{5}}^2\,\bint{0, \m_{\ind{3}}^2, \m_{\ind{4}}^2} \Big]\\
    &{-} \left(2 - \deltaMS\,\epsilon\right)
      \tintm{113}{\m_{\ind{3}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/104.tex <==
$\begin{aligned}
  & \cpl{SSVV}{\ind{1}, \ind{2}, \ind{3}, \ind{4}, 1}\,\times\\
  & \!\Big[
    4\,\cpl{VVVV}{\ind{3}, \ind{4}, \ind{5}, \ind{5}, 1}
     + \cpl{VVVV}{\ind{3}, \ind{4}, \ind{5}, \ind{5}, 2}
     + \cpl{VVVV}{\ind{3}, \ind{4}, \ind{5}, \ind{5}, 3}
    \Big]\,\times\\
  & \frac{1}{2} \,\bigg\{
    {-}\, \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right) \left[
      \aint{\m_{\ind{5}}^2} + \m_{\ind{5}}^2\,\bint{0, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \right]
  \!\!\bigg\}\\
  &{+}\,\cpl{SSVV}{\ind{1}, \ind{2}, \ind{3}, \ind{4}, 1}\,\times\\
  & \!\Big[
    \!\left(4 - 2\,\deltaMS\,\epsilon\right)
      \cpl{VVVV}{\ind{3}, \ind{4}, \ind{5}, \ind{5}, 1}
    + \cpl{VVVV}{\ind{3}, \ind{4}, \ind{5}, \ind{5}, 2}
    + \cpl{VVVV}{\ind{3}, \ind{4}, \ind{5}, \ind{5}, 3}
    \Big]\,\times\\
  & \frac{1}{2} \,\bigg\{
    \!\!\left(2 - \deltaMS\,\epsilon\right)
      \tintm{113}{\m_{\ind{3}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/105.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSS}{\ind{2}, \ind{5}, \ind{6}, 1}\,
    \cpl{SSSS}{\ind{3}, \ind{4}, \ind{5}, \ind{6}, 1}\,\times\\
  & \frac{1}{4}  \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \,\Big[
      \bint{p^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2} + \bint{p^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
      \Big]\\
    &{-}\, \tintm{1245}{\m_{\ind{3}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/106.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSVV}{\ind{3}, \ind{4}, \ind{5}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{5}, \ind{6}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon}\,\Big[
      2\,\bint{p^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
      + \left(2 - \deltaMS\,\epsilon\right) \bint{p^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \Big]\\
    &{-} \left(2 - \deltaMS\,\epsilon\right)
      \tintm{1245}{\m_{\ind{3}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/107.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{2}, \ind{5}, \ind{6}, 1}\,
    \cpl{SSVV}{\ind{3}, \ind{5}, \ind{4}, \ind{6}, 1}\,\times\\
  & \frac{1}{4} \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{3}{\epsilon}\,
      \yonesum{12}{[1]-[2]+3[6]}{\m_{\ind{3}}^2, \m_{\ind{4}}^2}
    + \ysum{1245}{4[1]-2[2]-[3]+4[6]}{\m_{\ind{3}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+} \left[\left(\ind{1},\ind{3},\ind{4}\right)\leftrightarrow\left(\ind{2},\ind{5},\ind{6}\right)\right]
\end{aligned}$


==> TeX/Selfs/108.tex <==
$\begin{aligned}
  &\left[\right]
\end{aligned}$

==> TeX/Selfs/109.tex <==
$\begin{aligned}
  & \cpl{SVV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
    \cpl{SVV}{\ind{2}, \ind{5}, \ind{6}, 1}\,\times\\
  & \!\Big[
    4\,\cpl{VVVV}{\ind{3}, \ind{4}, \ind{5}, \ind{6}, 1}
     + \cpl{VVVV}{\ind{3}, \ind{4}, \ind{5}, \ind{6}, 2}
     + \cpl{VVVV}{\ind{3}, \ind{4}, \ind{5}, \ind{6}, 3}
  \Big]\,\times\\
  &\frac{1}{2} \,\bigg\{
    \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right) \left[
      \bint{p^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
      + \bint{p^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \right]
  \bigg\}\\
  &{+}\,\cpl{SVV}{\ind{1}, \ind{3}, \ind{4}, 1}\,
        \cpl{SVV}{\ind{2}, \ind{5}, \ind{6}, 1}\,\times\\
  & \!\Big[
    \!\left(4 - 2\,\deltaMS\,\epsilon\right)
      \cpl{VVVV}{\ind{3}, \ind{4}, \ind{5}, \ind{6}, 1}
    + \cpl{VVVV}{\ind{3}, \ind{4}, \ind{5}, \ind{6}, 2}
    + \cpl{VVVV}{\ind{3}, \ind{4}, \ind{5}, \ind{6}, 3}
  \Big]\,\times\\
  & \frac{1}{2} \,\bigg\{
    {-} \left(2 - \deltaMS\,\epsilon\right)
      \tintm{1245}{\m_{\ind{3}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/110.tex <==
$\begin{aligned}
  & \m_{\ind{3}}\,\m_{\ind{4}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{5}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{4}, \ind{6}, 1}}\,
          \cpl{SSSS}{\ind{1}, \ind{2}, \ind{5}, \ind{6}, 1}\,\times\\
  & \bigg\{
    {-}\, \frac{1}{\epsilon}\,\bint{0, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    + \tintm{1134}{\m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}\\
  &{+}\,\Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{5}, 1}\,
              \cpl{FFS}{\ind{3}, \ind{4}, \ind{6}, 2}}\,
              \cpl{SSSS}{\ind{1}, \ind{2}, \ind{5}, \ind{6}, 1}\,\times\\
  &\frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \,\Big[
      {-}\, 2 \left(\m_{\ind{3}}^2 + \m_{\ind{4}}^2\right)
        \bint{0, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
      + \yoneint{11}{1}{\m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \Big]\\
    &{-}\, \ysum{1134}{[1]-[3]-[4]}{\m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/111.tex <==
$\begin{aligned}
  & \cpl{SSS}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SSS}{\ind{3}, \ind{4}, \ind{6}, 1}\,
    \cpl{SSSS}{\ind{1}, \ind{2}, \ind{5}, \ind{6}, 1}\,\times\\
  & \frac{1}{4} \,\bigg\{
    \frac{1}{\epsilon}\,\bint{0, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    - \tintm{1134}{\m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/112.tex <==
$\begin{aligned}
  & \cpl{SSSS}{\ind{1}, \ind{2}, \ind{5}, \ind{6}, 1}\,
    \cpl{SUU}{\ind{5}, -\ind{4}, \ind{3}, 1}\,
    \cpl{SUU}{\ind{6}, -\ind{3}, \ind{4}, 1}\,\times\\
  & \frac{1}{4} \,\bigg\{
    {-}\,\frac{1}{\epsilon}\,\bint{0, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    + \tintm{1134}{\m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/113.tex <==
$\begin{aligned}
  & \cpl{SSSS}{\ind{1}, \ind{2}, \ind{5}, \ind{6}, 1}\,
    \cpl{SSV}{\ind{3}, \ind{5}, \ind{4}, 1}\,
    \cpl{SSV}{\ind{3}, \ind{6}, \ind{4}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      & \aint{\m_{\ind{3}}^2}
        + 2 \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{4}}^2}
        + \left(\m_{\ind{3}}^2 + \m_{\ind{4}}^2\right)
          \bint{0, \m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
      &{+}\, 2\,\yoneint{11}{1}{\m_{\ind{5}}^2, \m_{\ind{6}}^2}
      \Big]
    \end{aligned}\\
    &{-}\, \ysum{1134}{2[1]+2[3]-[4]}{\m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/114.tex <==
$\begin{aligned}
  & \m_{\ind{3}}\,\m_{\ind{4}}\,
    \Real{\cpl{FFV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
          \cpl{FFV}{\ind{3}, \ind{4}, \ind{6}, 1}}\,
          \cpl{SSVV}{\ind{1}, \ind{2}, \ind{5}, \ind{6}, 1}\,\times\\
  & \bigg\{
    \frac{1}{\epsilon}
    \left(2 - \deltaMS\,\epsilon\right) \bint{0, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    - \left(2 - \deltaMS\,\epsilon\right)
      \tintm{1134}{\m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}\\
  &{+}\,\Real{\cpl{FFV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
              \cpl{FFV}{\ind{3}, \ind{4}, \ind{6}, 2}}\,
              \cpl{SSVV}{\ind{1}, \ind{2}, \ind{5}, \ind{6}, 1}\,\times\\
  & \frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \,\Big[
      \tfrac{1}{3} \left(3 - 2\, \deltaMS\,\epsilon\right)
        \yoneint{11}{1}{\m_{\ind{5}}^2, \m_{\ind{6}}^2}
      - 2 \left(2 - \deltaMS\,\epsilon\right)
        \m_{\ind{3}}^2\, \bint{0, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    \Big]\\
    &{-} \left(1 - \deltaMS\,\epsilon\right)
      \ysum{1134}{[1]-2[3]}{\m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+} \left[\ind{5}\leftrightarrow\ind{6}\right]
\end{aligned}$


==> TeX/Selfs/115.tex <==
$\begin{aligned}
  & \cpl{SSV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SSV}{\ind{3}, \ind{4}, \ind{6}, 1}\,
    \cpl{SSVV}{\ind{1}, \ind{2}, \ind{5}, \ind{6}, 1}\,\times\\
  & \frac{1}{4} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      &{-}\, \aint{\m_{\ind{3}}^2} - \aint{\m_{\ind{4}}^2}
        + \tfrac{1}{3} \left(3 - 2\, \deltaMS\,\epsilon\right)
          \yoneint{11}{1}{\m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
      &{-}\, \left(2 - \deltaMS\,\epsilon\right)
      \left(\m_{\ind{3}}^2 + \m_{\ind{4}}^2\right) \bint{0, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
      \Big]
    \end{aligned}\\
    &{-}\,\ysum{1134}{[1]-2[3]-2[4]}{\m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/116.tex <==
$\begin{aligned}
  & \cpl{SSSS}{\ind{1}, \ind{2}, \ind{5}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{5}, \ind{3}, \ind{4}, 1}\,
    \cpl{SVV}{\ind{6}, \ind{3}, \ind{4}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{
    \frac{2}{\epsilon}\,\bint{0, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    - \left(2 - \deltaMS\,\epsilon\right)
      \tintm{1134}{\m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/117.tex <==
$\begin{aligned}
  & \begin{aligned}[t] \!\Big[
    & \cpl{SSVV}{\ind{1}, \ind{2}, \ind{5}, \ind{6}, 1}\,
      \cpl{UUV}{-\ind{3}, \ind{4}, \ind{6}, 1}\,
      \cpl{UUV}{-\ind{4}, \ind{3}, \ind{5}, 1}\\
    &{+}\,\cpl{SSVV}{\ind{1}, \ind{2}, \ind{5}, \ind{6}, 1}\,
          \cpl{UUV}{\ind{3}, -\ind{4}, \ind{6}, 2}\,
          \cpl{UUV}{\ind{4}, -\ind{3}, \ind{5}, 2}
    \Big]\,\times
  \end{aligned}\\
  & \frac{1}{8} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \left[
      \tfrac{1}{3} \left(3 - \deltaMS\,\epsilon\right)
        \yoneint{11}{1}{\m_{\ind{5}}^2, \m_{\ind{6}}^2}
      - \left(2 - \deltaMS\,\epsilon\right)
        \left(\m_{\ind{3}}^2 + \m_{\ind{4}}^2\right)
        \bint{0, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
      \right]\\
    &{-}\,\ysum{1134}{[1]-[3]-[4]}{\m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/118.tex <==
$\begin{aligned}
  & \cpl{SSVV}{\ind{1}, \ind{2}, \ind{5}, \ind{6}, 1}\,
    \cpl{SVV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SVV}{\ind{3}, \ind{4}, \ind{6}, 1}\,\times\\
  & \!\bigg\{
    {-}\, \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
      \bint{0, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
    + \left(2 - \deltaMS\,\epsilon\right)
      \tintm{1134}{\m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/119.tex <==
$\begin{aligned}
  & \cpl{SSVV}{\ind{1}, \ind{2}, \ind{5}, \ind{6}, 1}\,
    \cpl{VVV}{\ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{VVV}{\ind{3}, \ind{4}, \ind{6}, 1}\,\times\\
  & \frac{1}{4} \begin{aligned}[t] \,\bigg\{
    &{-} \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      & \!\left(2 - \deltaMS\,\epsilon\right) \begin{aligned}[t] \big[
        & 9\,\aint{\m_{\ind{3}}^2} + 9\,\aint{\m_{\ind{4}}^2}
          - \yoneint{11}{1}{\m_{\ind{5}}^2, \m_{\ind{6}}^2}\\
        &{+}\, 9 \left(\m_{\ind{3}}^2 + \m_{\ind{4}}^2\right)
          \bint{0, \m_{\ind{5}}^2, \m_{\ind{6}}^2}
        \big]
      \end{aligned}\\
      & \tfrac{11}{3} \left(3 - 2\, \deltaMS\,\epsilon\right)
        \yoneint{11}{1}{\m_{\ind{5}}^2, \m_{\ind{6}}^2}
      \Big]
    \end{aligned}\\
    &{+}\, 3 \left(3 - 2\, \deltaMS\,\epsilon\right)
      \ysum{1134}{[1]+[3]+[4]}{\m_{\ind{5}}^2, \m_{\ind{6}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Selfs/120.tex <==
$\begin{aligned}
  & \cpl{SSSS}{\ind{1}, \ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SSSS}{\ind{2}, \ind{3}, \ind{4}, \ind{5}, 1}\,\times\\
  & \frac{1}{6} \,\bigg\{
    \frac{1}{\epsilon} \,\Big[
      \aint{\m_{\ind{3}}^2} + \aint{\m_{\ind{4}}^2} + \aint{\m_{\ind{5}}^2}
    \Big]
    - \tintm{234}{\m_{\ind{3}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Selfs/121.tex <==
$\begin{aligned}
  & \cpl{SSVV}{\ind{1}, \ind{3}, \ind{4}, \ind{5}, 1}\,
    \cpl{SSVV}{\ind{2}, \ind{3}, \ind{4}, \ind{5}, 1}\,\times\\
  & \begin{aligned}[t] \bigg\{
    & \frac{1}{\epsilon} \,\Big[
      2\,\aint{\m_{\ind{3}}^2}
      + \left(2 - \deltaMS\,\epsilon\right)
        \left[\aint{\m_{\ind{4}}^2} + \aint{\m_{\ind{5}}^2}\right]\!\Big]\\
    &{-} \left(2 - \deltaMS\,\epsilon\right)
      \tintm{234}{\m_{\ind{3}}^2, \m_{\ind{4}}^2, \m_{\ind{5}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/01.tex <==
$\begin{aligned}
  &\cpl{SSS}{\ind{1}, \ind{2}, \ind{3}, 1}\,\cpl{SSSS}{\ind{2}, \ind{3}, \ind{4}, \ind{4}, 1}\,\times\\
  &\frac{1}{4} \,\bigg\{
  \frac{1}{\epsilon}\, \Big[ \aint{\m_{\ind{4}}^2}
    + \m_{\ind{4}}^2\,\bint{0, \m_{\ind{2}}^2, \m_{\ind{3}}^2} \Big]
  - \tintm{113}{\m_{\ind{2}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Tads/02.tex <==
$\begin{aligned}
  &\cpl{SSS}{\ind{1}, \ind{2}, \ind{3}, 1}\,\cpl{SSVV}{\ind{2}, \ind{3}, \ind{4}, \ind{4}, 1}\,\times\\
  &\frac{1}{2} \begin{aligned}[t] \,\bigg\{
  &{-}\, \frac{1}{\epsilon}\,\Big[
    2\,\m_{\ind{4}}^2\,\bint{0, \m_{\ind{2}}^2, \m_{\ind{3}}^2}
    + \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{4}}^2} \Big]\\
  &{+} \left(2 - \deltaMS\,\epsilon\right)
    \tintm{113}{\m_{\ind{2}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/03.tex <==
$\begin{aligned}
  &\cpl{SSVV}{\ind{4}, \ind{4}, \ind{2}, \ind{3}, 1}\,\cpl{SVV}{\ind{1}, \ind{2}, \ind{3}, 1}\,\times\\
  &\frac{1}{2} \begin{aligned}[t] \,\bigg\{
    &\frac{1}{\epsilon} \,\Big[ 2\,\aint{\m_{\ind{4}}^2}
      + \left(2 - \deltaMS\,\epsilon\right)
      \m_{\ind{4}}^2\,\bint{0, \m_{\ind{2}}^2, \m_{\ind{3}}^2} \Big]\\
    &{-} \left(2 - \deltaMS\,\epsilon\right)
      \tintm{113}{\m_{\ind{2}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/04.tex <==
$\begin{aligned}
  & \cpl{SVV}{\ind{1}, \ind{2}, \ind{3}, 1}\,\times\\
  & \!\Big[
    4\,\cpl{VVVV}{\ind{2}, \ind{3}, \ind{4}, \ind{4}, 1}
     + \cpl{VVVV}{\ind{2}, \ind{3}, \ind{4}, \ind{4}, 2}
     + \cpl{VVVV}{\ind{2}, \ind{3}, \ind{4}, \ind{4}, 3}
    \Big]\,\times\\
  & \frac{1}{2} \,\bigg\{
    {-}\,\frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right) \Big[
      \aint{\m_{\ind{4}}^2} + \m_{\ind{4}}^2\,\bint{0, \m_{\ind{2}}^2, \m_{\ind{3}}^2}
    \Big]
  \!\bigg\}\\
  & \cpl{SVV}{\ind{1}, \ind{2}, \ind{3}, 1}\,\times\\
  & \!\Big[
    \!\left(4 - 2\,\deltaMS\,\epsilon\right)
      \cpl{VVVV}{\ind{2}, \ind{3}, \ind{4}, \ind{4}, 1}
    + \cpl{VVVV}{\ind{2}, \ind{3}, \ind{4}, \ind{4}, 2}
    + \cpl{VVVV}{\ind{2}, \ind{3}, \ind{4}, \ind{4}, 3}
    \Big]\,\times\\
  & \frac{1}{2} \,\bigg\{
    \!\!\left(2 - \deltaMS\,\epsilon\right)
      \tintm{113}{\m_{\ind{2}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Tads/05.tex <==
$\begin{aligned}
  & \m_{\ind{2}}\,\m_{\ind{3}}\,\m_{\ind{5}}\,
    \Real{\cpl{FFS}{\ind{2}, \ind{3}, \ind{4}, 1}\,
          \cpl{FFS}{\ind{2}, \ind{5}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{5}, \ind{4}, 1}}\,\times\\
  & 2\,\bigg\{
    {-}\, \frac{1}{\epsilon}\, \bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}
    + \tintm{1134}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}\\
  &{+}\,\m_{\ind{3}}\,
    \Real{\cpl{FFS}{\ind{2}, \ind{3}, \ind{4}, 1}\,
          \cpl{FFS}{\ind{2}, \ind{5}, \ind{1}, 2}\,
          \cpl{FFS}{\ind{3}, \ind{5}, \ind{4}, 1}}\,\times\\
  & 2 \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon} \,\Big[
        \aint{\m_{\ind{3}}^2} + \aint{\m_{\ind{4}}^2}
        + \yoneint{11}{1}{\m_{\ind{2}}^2, \m_{\ind{5}}^2}
        \Big]\\
    &{+}\, \yint{1134}{1}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+}\,\Big[\m_{\ind{2}} + \m_{\ind{5}}\Big]\,
    \Real{\cpl{FFS}{\ind{2}, \ind{3}, \ind{4}, 1}\,
          \cpl{FFS}{\ind{2}, \ind{5}, \ind{1}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{5}, \ind{4}, 2}}\,\times\\
    & \begin{aligned}[t] \bigg\{
      &{-}\, \frac{1}{\epsilon} \,\Big[
        2\, \aint{\m_{\ind{4}}^2} + \yoneint{11}{1}{\m_{\ind{2}}^2, \m_{\ind{5}}^2}
        \Big]
      + \ysum{1134}{[1]+[3]-[4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/06.tex <==
$\begin{aligned}
  & \m_{\ind{3}}\,\m_{\ind{4}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{2}, 1}\,
          \cpl{FFS}{\ind{3}, \ind{4}, \ind{5}, 1}}\,
          \cpl{SSS}{\ind{1}, \ind{2}, \ind{5}, 1}\,\times\\
  & \bigg\{
  {-}\, \frac{1}{\epsilon}\,\bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}
   + \tintm{1134}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}\\
  &{+}\,\Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{2}, 1}\,
              \cpl{FFS}{\ind{3}, \ind{4}, \ind{5}, 2}}\,
              \cpl{SSS}{\ind{1}, \ind{2}, \ind{5}, 1}\,\times\\
  &\frac{1}{2} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \,\Big[ \yoneint{11}{1}{\m_{\ind{2}}^2,\m_{\ind{5}}^2}
      - 2 \left(\m_{\ind{3}}^2 + \m_{\ind{4}}^2\right)
        \bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2} \Big]\\
    &{-}\, \ysum{1134}{[1]-[3]-[4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/07.tex <==
$\begin{aligned}
  &\cpl{SSS}{\ind{1}, \ind{2}, \ind{5}, 1}\,\cpl{SSS}{\ind{2}, \ind{3}, \ind{4}, 1}\,\cpl{SSS}{\ind{3}, \ind{4}, \ind{5}, 1}\,\times\\
  &\frac{1}{4} \,\bigg\{
  \frac{1}{\epsilon}\,\bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}
  - \tintm{1134}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Tads/08.tex <==
$\begin{aligned}
  &\cpl{SSS}{\ind{1}, \ind{2}, \ind{5}, 1}\,
   \cpl{SUU}{\ind{2}, -\ind{3}, \ind{4}, 1}\,
   \cpl{SUU}{\ind{5}, -\ind{4}, \ind{3}, 1}\,\times\\
  &\frac{1}{4} \,\bigg\{
    {-}\, \frac{1}{\epsilon}\,\bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}
    + \tintm{1134}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Tads/09.tex <==
$\begin{aligned}
  &\cpl{SUU}{\ind{1}, -\ind{5}, \ind{2}, 1}\,
   \cpl{SUU}{\ind{3}, -\ind{2}, \ind{4}, 1}\,
   \cpl{SUU}{\ind{3}, -\ind{4}, \ind{5}, 1}\,\times\\
  &\frac{1}{2} \,\bigg\{
    {-}\, \frac{1}{\epsilon}\,\bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}
    + \tintm{1134}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Tads/10.tex <==
$\begin{aligned}
  & \m_{\ind{2}}\,\m_{\ind{3}}\,\m_{\ind{5}}\,
    \Real{\cpl{FFS}{\ind{2}, \ind{5}, \ind{1}, 1}\,
          \cpl{FFV}{\ind{2}, \ind{3}, \ind{4}, 2}\,
          \cpl{FFV}{\ind{3}, \ind{5}, \ind{4}, 1}}\,\times\\
  & 4 \begin{aligned}[t] \,\bigg\{
    & \frac{2}{\epsilon}\,\bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}
      - \left(2 - \deltaMS\,\epsilon\right)
        \tintm{1134}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+}\,\m_{\ind{3}}\,
    \Real{\cpl{FFS}{\ind{2}, \ind{5}, \ind{1}, 1}\,
          \cpl{FFV}{\ind{2}, \ind{3}, \ind{4}, 1}\,
          \cpl{FFV}{\ind{3}, \ind{5}, \ind{4}, 2}}\,\times\\
  & 4 \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \,\Big[
      2\,\aint{\m_{\ind{3}}^2} + 2\,\yoneint{11}{1}{\m_{\ind{2}}^2, \m_{\ind{5}}^2}
      + \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{4}}^2}
      \Big]\\
    &{-} \left(2 - \deltaMS\,\epsilon\right)
        \yint{1134}{1}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}\\
  &{+} \begin{aligned}[t] \,\Big[
    & \m_{\ind{2}}\,
      \Real{\cpl{FFS}{\ind{2}, \ind{5}, \ind{1}, 1}\,
            \cpl{FFV}{\ind{2}, \ind{3}, \ind{4}, 2}\,
            \cpl{FFV}{\ind{3}, \ind{5}, \ind{4}, 2}}\\
    &{+}\, \m_{\ind{5}}\,
      \Real{\cpl{FFS}{\ind{2}, \ind{5}, \ind{1}, 1}\,
            \cpl{FFV}{\ind{2}, \ind{3}, \ind{4}, 1}\,
            \cpl{FFV}{\ind{3}, \ind{5}, \ind{4}, 1}}
      \Big]\,\times
  \end{aligned}\\
  & 2 \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon} \,\Big[
        \yoneint{11}{1}{\m_{\ind{2}}^2, \m_{\ind{5}}^2}
        + \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{4}}^2}
        \Big]\\
    &{+} \left(1 - \deltaMS\,\epsilon\right)
    \ysum{1134}{[1] + [3] - [4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/11.tex <==
$\begin{aligned}
  & \m_{\ind{3}}\,
    \Real{\cpl{FFS}{\ind{3}, \ind{4}, \ind{2}, 1}\,
          \cpl{FFV}{\ind{3}, \ind{4}, \ind{5}, 2}}\,
          \cpl{SSV}{\ind{1}, \ind{2}, \ind{5}, 1}\,\times\\
  & \bigg\{
    \frac{1}{\epsilon} \,\Big[
      2\, \aint{\m_{\ind{3}}^2} + \yoneint{11}{1}{\m_{\ind{2}}^2, \m_{\ind{5}}^2}
    \Big]
    - \ysum{1134}{[1] - [3] + [4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}\\
  &{+} \left[\ind{3}\leftrightarrow\ind{4}\right]
\end{aligned}$


==> TeX/Tads/12.tex <==
$\begin{aligned}
  &\cpl{SSS}{\ind{2}, \ind{3}, \ind{4}, 1}\,\cpl{SSV}{\ind{1}, \ind{2}, \ind{5}, 1}\,\cpl{SSV}{\ind{3}, \ind{4}, \ind{5}, 1}\,\times\\
  &\frac{1}{2} \,\bigg\{
    \frac{1}{\epsilon} \,\Big[\aint{\m_{\ind{3}}^2} - \aint{\m_{\ind{4}}^2}\Big]
    - \ysum{1134}{[3]-[4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Tads/13.tex <==
$\begin{aligned}
  &\cpl{SSS}{\ind{1}, \ind{2}, \ind{5}, 1}\,\cpl{SSV}{\ind{2}, \ind{3}, \ind{4}, 1}\,\cpl{SSV}{\ind{3}, \ind{5}, \ind{4}, 1}\,\times\\
  &\frac{1}{2} \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      &\aint{\m_{\ind{3}}^2}
        + 2 \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{4}}^2}\\
      &{+} \left(\m_{\ind{3}}^2 + \m_{\ind{4}}^2\right)
          \bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}
        + 2\,\yoneint{11}{1}{\m_{\ind{2}}^2,\m_{\ind{5}}^2}
      \Big]
    \end{aligned}\\
    &{+}\, \ysum{1134}{2[1]-[3]+2[4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/14.tex <==
% $\begin{aligned}
%   & \cpl{SSV}{\ind{1}, \ind{2}, \ind{5}, 1}\,
%     \cpl{SUU}{\ind{2}, -\ind{3}, \ind{4}, 1}\,
%     \cpl{UUV}{-\ind{4}, \ind{3}, \ind{5}, 1}\,\times\\
%   & \frac{1}{4} \,\bigg\{
%     \frac{1}{\epsilon}\,\Big[
%       2\,\aint{\m_{\ind{3}}^2} + \yoneint{11}{1}{\m_{\ind{2}}^2, \m_{\ind{5}}^2}
%     \Big]
%     - \ysum{1134}{[1]-[3]+[4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
%   \!\bigg\}\\    
%   &{+} \left[\ind{3}\leftrightarrow\ind{4}\right]
% \end{aligned}$
$\begin{aligned}
  & \cpl{SSV}{\ind{1}, \ind{2}, \ind{5}, 1}\,
    \cpl{SUU}{\ind{2}, -\ind{3}, \ind{4}, 1}\,
    \cpl{UUV}{-\ind{4}, \ind{3}, \ind{5}, 1}\,\times\\
  & \frac{1}{2} \,\bigg\{ %% added factor of 2
    \frac{1}{\epsilon}\,\Big[
      2\,\aint{\m_{\ind{3}}^2} + \yoneint{11}{1}{\m_{\ind{2}}^2, \m_{\ind{5}}^2}
    \Big]
    - \ysum{1134}{[1]-[3]+[4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
%  &{+} \left[\ind{3}\leftrightarrow\ind{4}\right]
\end{aligned}$


==> TeX/Tads/15.tex <==
$\begin{aligned}
  & \begin{aligned}[t] \Big[
      & \cpl{SUU}{\ind{1}, -\ind{5}, \ind{2}, 1}\,
        \cpl{UUV}{-\ind{2}, \ind{3}, \ind{4}, 1}\,
        \cpl{UUV}{-\ind{3}, \ind{5}, \ind{4}, 1}\\
      &{+}\,\cpl{SUU}{\ind{1}, \ind{5}, -\ind{2}, 1}\,
            \cpl{UUV}{\ind{2}, -\ind{3}, \ind{4}, 2}\,
            \cpl{UUV}{\ind{3}, -\ind{5}, \ind{4}, 2}
      \Big]
    \end{aligned}\\
  & \frac{1}{4} \begin{aligned}[t] \,\bigg\{
      & \frac{1}{\epsilon} \,\Big[
        \yoneint{11}{1}{\m_{\ind{2}}^2, \m_{\ind{5}}^2}
        + \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{4}}^2}
      \Big]\\
    &{-}\, \ysum{1134}{[1] + [3] - [4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/16.tex <==
$\begin{aligned}
  & \m_{\ind{3}}\,\m_{\ind{4}}\,
    \Real{\cpl{FFV}{\ind{3}, \ind{4}, \ind{2}, 1}\,
          \cpl{FFV}{\ind{3}, \ind{4}, \ind{5}, 1}}\,
          \cpl{SVV}{\ind{1}, \ind{2}, \ind{5}, 1}\,\times\\
  & 2\,\bigg\{
    \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
      \bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}
    - \left(2 - \deltaMS\,\epsilon\right)
      \tintm{1134}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}\\
  &{+}\,\Real{\cpl{FFV}{\ind{3}, \ind{4}, \ind{2}, 1}\,
    \cpl{FFV}{\ind{3}, \ind{4}, \ind{5}, 2}}\,
    \cpl{SVV}{\ind{1}, \ind{2}, \ind{5}, 1}\,\times\\
  & \begin{aligned}[t] \bigg\{
    &\frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      &{-} \left(2 - \deltaMS\,\epsilon\right)
          \left(\m_{\ind{3}}^2 + \m_{\ind{4}}^2\right)
          \bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}\\
      &{+}\, \tfrac{1}{3} \left(3 - 2\, \deltaMS\,\epsilon\right)
        \yoneint{11}{1}{\m_{\ind{2}}^2,\m_{\ind{5}}^2}
      \Big]
    \end{aligned}\\
    &{-} \left(1 - \deltaMS\,\epsilon\right)
        \ysum{1134}{[1]-[3]-[4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/17.tex <==
$\begin{aligned}
  &\cpl{SSV}{\ind{3}, \ind{4}, \ind{2}, 1}\,\cpl{SSV}{\ind{3}, \ind{4}, \ind{5}, 1}\,\cpl{SVV}{\ind{1}, \ind{2}, \ind{5}, 1}\,\times\\
  &\frac{1}{4} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \begin{aligned}[t] \,\Big[
      &{-}\, \aint{\m_{\ind{3}}^2} - \aint{\m_{\ind{4}}^2}
        + \tfrac{1}{3} \left(3 - 2\, \deltaMS\,\epsilon\right)
          \yoneint{11}{1}{\m_{\ind{2}}^2,\m_{\ind{5}}^2}\\
      &{-}\, 2 \left(2 - \deltaMS\,\epsilon\right)
          \left(\m_{\ind{3}}^2 + \m_{\ind{4}}^2\right)
          \bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}
      \Big]
    \end{aligned}\\
    &{-} \,\ysum{1134}{[1]-2[3]-2[4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/18.tex <==
$\begin{aligned}
  &\cpl{SSV}{\ind{1}, \ind{2}, \ind{5}, 1}\,\cpl{SSV}{\ind{2}, \ind{3}, \ind{4}, 1}\,\cpl{SVV}{\ind{3}, \ind{4}, \ind{5}, 1}\,\times\\
  &\frac{1}{2} \begin{aligned}[t] \,\bigg\{
    &\frac{1}{\epsilon} \,\Big[
      2\,\aint{\m_{\ind{3}}^2} + 3\,\yoneint{11}{1}{\m_{\ind{2}}^2,\m_{\ind{5}}^2}
      + 2 \left(2 - \deltaMS\,\epsilon\right) \aint{\m_{\ind{4}}^2}
      \Big]\\
    &{-}\, \ysum{1134}{3[1]-[3]+[4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/19.tex <==
$\begin{aligned}
  &\cpl{SSS}{\ind{1}, \ind{2}, \ind{5}, 1}\,\cpl{SVV}{\ind{2}, \ind{3}, \ind{4}, 1}\,\cpl{SVV}{\ind{5}, \ind{3}, \ind{4}, 1}\,\times\\
  &\frac{1}{2} \,\bigg\{
    \frac{2}{\epsilon}\,\bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}
    - \left(2 - \deltaMS\,\epsilon\right)
      \tintm{1134}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Tads/20.tex <==
$\begin{aligned}
  & \begin{aligned}[t] \Big[
    & \cpl{SVV}{\ind{1}, \ind{2}, \ind{5}, 1}\,
      \cpl{UUV}{-\ind{3}, \ind{4}, \ind{2}, 1}\,
      \cpl{UUV}{-\ind{4}, \ind{3}, \ind{5}, 1}\\
    &{+}\,\cpl{SVV}{\ind{1}, \ind{2}, \ind{5}, 1}\,
          \cpl{UUV}{\ind{3}, -\ind{4}, \ind{2}, 2}\,
          \cpl{UUV}{\ind{4}, -\ind{3}, \ind{5}, 2}
    \Big]\,\times
  \end{aligned}\\
  & \frac{1}{8} \begin{aligned}[t] \,\bigg\{
    & \frac{1}{\epsilon} \left[
      \tfrac{1}{3} \left(3 - \deltaMS\,\epsilon\right)
        \yoneint{11}{1}{\m_{\ind{2}}^2, \m_{\ind{5}}^2}
      - \left(2 - \deltaMS\,\epsilon\right)
        \left(\m_{\ind{3}}^2 + \m_{\ind{4}}^2\right)
        \bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}
      \right]\\
    &{-}\, \ysum{1134}{[1] - [3] - [4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/21.tex <==
$\begin{aligned}
  &\cpl{SVV}{\ind{1}, \ind{2}, \ind{5}, 1}\,\cpl{SVV}{\ind{3}, \ind{2}, \ind{4}, 1}\,\cpl{SVV}{\ind{3}, \ind{4}, \ind{5}, 1}\,\times\\
  &\bigg\{
  {-}\, \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
    \bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}
  + \left(2 - \deltaMS\,\epsilon\right)
    \tintm{1134}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Tads/22.tex <==
$\begin{aligned}
  &\cpl{SSV}{\ind{1}, \ind{2}, \ind{5}, 1}\,\cpl{SVV}{\ind{2}, \ind{3}, \ind{4}, 1}\,\cpl{VVV}{\ind{3}, \ind{4}, \ind{5}, 1}\,\times\\
  &\frac{1}{4} \begin{aligned}[t] \,\bigg\{
    &{-}\,\frac{3}{\epsilon} \left(2 - \deltaMS\,\epsilon\right) \Big[
      \aint{\m_{\ind{3}}^2} - \aint{\m_{\ind{4}}^2} \Big]\\
    &{+}\, 2 \left(3 - 2\, \deltaMS\,\epsilon\right)
      \ysum{1134}{[3]-[4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/23.tex <==
$\begin{aligned}
  &\cpl{SVV}{\ind{1}, \ind{2}, \ind{5}, 1}\,\cpl{VVV}{\ind{2}, \ind{3}, \ind{4}, 1}\,\cpl{VVV}{\ind{3}, \ind{4}, \ind{5}, 1}\,\times\\
  &\frac{1}{4} \begin{aligned}[t] \,\bigg\{
    &{-}\, \frac{1}{\epsilon} \left(2 - \deltaMS\,\epsilon\right)
      \begin{aligned}[t] \Big[
      & 9\, \aint{\m_{\ind{3}}^2} + 9\, \aint{\m_{\ind{4}}^2}\\
      &{+}\, 9 \left(\m_{\ind{3}}^2 + \m_{\ind{4}}^2\right)
          \bint{0, \m_{\ind{2}}^2, \m_{\ind{5}}^2}
        - \yoneint{11}{1}{\m_{\ind{2}}^2, \m_{\ind{5}}^2}
      \Big]
      \end{aligned}\\
      &{-}\, \frac{11}{3\,\epsilon} \left(3 - 2\, \deltaMS\,\epsilon\right)
          \yoneint{11}{1}{\m_{\ind{2}}^2, \m_{\ind{5}}^2}\\
      &{+}\, 3 \left(3 - 2\, \deltaMS\,\epsilon\right)
          \ysum{1134}{[1]+[3]+[4]}{\m_{\ind{2}}^2, \m_{\ind{5}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}
\end{aligned}$


==> TeX/Tads/24.tex <==
$\begin{aligned}
  &\cpl{SSS}{\ind{2}, \ind{3}, \ind{4}, 1}\,\cpl{SSSS}{\ind{1}, \ind{2}, \ind{3}, \ind{4}, 1}\,\times\\
  &\frac{1}{6} \,\bigg\{
  \frac{1}{\epsilon} \,\Big[
    \aint{\m_{\ind{2}}^2} + \aint{\m_{\ind{3}}^2} + \aint{\m_{\ind{4}}^2}
    \Big]
  - \tintm{134}{\m_{\ind{2}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
  \!\bigg\}
\end{aligned}$


==> TeX/Tads/25.tex <==
$\begin{aligned}
  &\cpl{SSVV}{\ind{1}, \ind{2}, \ind{3}, \ind{4}, 1}\,\cpl{SVV}{\ind{2}, \ind{3}, \ind{4}, 1}\,\times\\
  &\begin{aligned}[t] \bigg\{
    & \frac{1}{\epsilon} \,\Big[ 2\,\aint{\m_{\ind{2}}^2}
      + \left(2 - \deltaMS\,\epsilon\right) \left[ \aint{\m_{\ind{3}}^2}
        + \aint{\m_{\ind{4}}^2}\right]
      \!\Big]\\
    &{-} \left(2 - \deltaMS\,\epsilon\right)
         \tintm{134}{\m_{\ind{2}}^2, \m_{\ind{3}}^2, \m_{\ind{4}}^2}
    \!\bigg\}
  \end{aligned}     
\end{aligned}$


==> definitions.tex <==
\input{unicode}

\normalem

\makeatletter
\patchcmd{\upbracefill}{\m@th}{\scriptstyle\m@th}{}{}
\patchcmd{\upbracefill}{$\braceld$}{$\scriptstyle\braceld$}{}{}
\patchcmd{\upbracefill}{\bracelu}{\bracelu\mkern-1mu}{}{}
\patchcmd{\upbracefill}{\hfill\braceru}{\hfill\mkern-1mu\braceru}{}{}
\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\makeatother

\newlength{\floatwidth}
\setlength{\floatwidth}{\dimexpr(\textwidth-1cm)\relax}

\def\bra{\langle}
\def\ket{\rangle}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\nn{\nonumber}
\def\ov{\overline}
\def\blog{\overline{\log}}
\def\bA{\mathbf{A}}
\def\bI{\mathbf{I}}
\def\bB{\mathbf{B}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bM{\mathbf{M}}
\def\OV{\mathcal{O}^{(V)}}
\def\OS{\mathcal{O}^{(S)}}
\def\llog{\overline{\log}}
\newcommand{\fin}[1]{\mathrm{Fin}{\left[#1\right]}}



%\def\website{\text{\url{www.OurWebSite.com}}\xspace}
%\def\ourcode{\texttt{TLDR}\xspace}
\def\website{\text{\url{http://tldr.hepforge.org}}\xspace}
\def\websiteB{\text{\url{https://launchpad.net/tldr}}\xspace}
\def\ourcode{{\tt TLDR}\xspace}


\def\lag{\mathcal{L}}
\def\lagr{\mathcal{L}}
\def\veff{V_\text{eff}}
\def\vtree{V^{(0)}}
\def\vone{V^{(1)}}
\newcommand{\veffr}{\hat{V}_{\text{eff}}}
\newcommand{\gbm}{m_G^2}
\newcommand{\voner}{\hat{V}^{(1)}}
\newcommand{\vtwor}{\hat{V}^{(2)}}
\newcommand{\vtwo}{V^{(2)}}
\newcommand{\vtwos}{V^{(2)}_S}

\def\selfdir{../Notes/FG/Selfs}

\def\igtad[#1][#2]{%
\begin{minipage}[c]{.3\textwidth}%
\phantomsection%
\label{tad:#1}%
\vspace{.5ex}\includegraphics[width=#2\textwidth]{Figs/Tads/#1}\vspace{.5ex}%
\end{minipage}%
}%
\def\igself[#1]{%
\begin{minipage}[c]{.3\textwidth}%
\phantomsection%
\label{se:#1}%
\vspace{.5ex}\includegraphics[width=\textwidth]{Figs/Selfs/#1}\vspace{.5ex}%
\end{minipage}%
}%
\def\restad[#1]{%
\begin{minipage}[c]{.6\textwidth}%
\small
\vspace{1ex}\scalebox{.9}{\input{TeX/Tads/#1}}\vspace{1ex}%
\end{minipage}%
}%
\def\resself[#1]{%
\begin{minipage}[c]{.6\textwidth}%
\small
\vspace{1ex}\scalebox{.9}{\input{TeX/Selfs/#1}}\vspace{1ex}%
\end{minipage}%
}%

\def\twomat[#1,#2][#3,#4]{\left( \begin{array}{cc} #1 & #2 \\ #3 & #4 \end{array} \right)}
\def\threemat[#1,#2,#3][#4,#5,#6][#7,#8,#9]{\left( \begin{array}{ccc} #1 & #2 & #3\\ #4 & #5 & #6 \\ #7 & #8 & #9 \end{array} \right)}
\def\twovec[#1,#2]{\left( \begin{array}{c} #1  \\ #2 \end{array} \right)}
\def\thv[#1,#2,#3]{\left( \begin{array}{c} #1 \\ #2 \\ #3 \end{array} \right)}
\def\twv[#1,#2]{\left( \begin{array}{c} #1 \\ #2 \end{array} \right)}

\newcommand{\minitab}[2][l]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\newcommand{\IE}{\textit{i.\,e.}\xspace}
\newcommand{\EG}{\textit{e.\,g.}\xspace}
\newcommand{\refeq}[1]{Eq.\,\eqref{#1}}
\newcommand{\refeqs}[1]{Eqs.\,\eqref{#1}}
\newcommand{\sect}[1]{Sect.\,\ref{#1}}
\newcommand{\appx}[1]{Appx.\,\ref{#1}}
\newcommand{\fig}[1]{Fig.\,\ref{#1}}
\newcommand{\tab}[1]{Tab.\,\ref{#1}}
\newcommand{\citere}[1]{Ref.\,\cite{#1}}
\newcommand{\citeres}[1]{Refs.\,\cite{#1}}
\newcommand{\simord}{\mathord{\sim}\,}
\newcommand{\simeqord}{\mathord{\simeq}\,}
\newcommand{\lsimord}{\mathord{\lesssim}\,}
\newcommand{\gsimord}{\mathord{\gtrsim}\,}
\newcommand{\leqord}{\mathord{\leq}\,}
\newcommand{\yint}[3]{Y_{#1}^{[#2]}\ifthenelse{\isempty{#3}}{}{{\left(#3\right)}}}
\newcommand{\ysum}[3]{Y_{#1}^{#2}\ifthenelse{\isempty{#3}}{}{{\left(#3\right)}}}
\newcommand{\yonesum}[3]{{^0}Y_{#1}^{#2}\ifthenelse{\isempty{#3}}{}{{\left(#3\right)}}}
\newcommand{\tint}[2]{\ifthenelse{\isempty{#2}}{T_{#1}}{T_{#1}^{\left|#2\right.}}}
\newcommand{\tintm}[2]{T_{#1}{\left(#2\right)}}
\newcommand{\toneint}[2]{\ifthenelse{\isempty{#2}}{{^0}T_{#1}}{^0T^{\left|#2\right.}_{#1}}}
\newcommand{\toneintm}[2]{{^0}T_{#1}{\left(#2\right)}}
\newcommand{\yoneint}[3]{{^0}Y_{#1}^{[#2]}\ifthenelse{\isempty{#3}}{}{{\left(#3\right)}}}
\newcommand{\bint}[1]{B_{0}\ifthenelse{\isempty{#1}}{}{{\left(#1\right)}}}
\newcommand{\aint}[1]{A_{0}\ifthenelse{\isempty{#1}}{}{{\left(#1\right)}}}
\newcommand{\binteps}[2]{\ifthenelse{\isempty{#2}}{B_{0}^{\left|#1\right.}}{B_{0}^{\left|#1\right.}{\!\left(#2\right)}}}
\newcommand{\ainteps}[2]{A_{0}^{\left|#1\right.}{\!\left(#2\right)}}
\newcommand{\mydelta}[1]{\Delta_{#1}}
\newcommand{\mygamma}[1]{\Gamma{\left(#1\right)}}
\newcommand{\mybrace}[2]{\smash{\underbrace{\scriptstyle #1}_{#2}}}
\newcommand{\myu}[1]{u_{#1}}
\newcommand{\FeynArts}{\texttt{FeynArts}\xspace}
\newcommand{\FormCalc}{\texttt{FormCalc}\xspace}
\newcommand{\TSIL}{\texttt{TSIL}\xspace}
\newcommand{\TARCER}{\texttt{TARCER}\xspace}
\newcommand{\SARAH}{\texttt{SARAH}\xspace}
\newcommand{\SMH}{\texttt{SMH}\xspace}
\newcommand{\mr}{\texttt{mr}\xspace}
\newcommand{\SMDR}{\texttt{SMDR}\xspace}
\newcommand{\Himalaya}{\texttt{Himalaya}\xspace}
\newcommand{\OneCalc}{\texttt{OneCalc}\xspace}
\newcommand{\TwoCalc}{\texttt{TwoCalc}\xspace}
\newcommand{\CP}{\ensuremath{\mathcal{CP}}\xspace}
\newcommand{\MS}{\ensuremath{\overline{\text{MS}}}\xspace}
\newcommand{\DR}{\ensuremath{\overline{\text{DR}}}\xspace}
\newcommand{\deltaMS}{\delta_{\scriptscriptstyle\MS}}
\newcommand{\ind}[1]{\text{i}#1}
\newcommand{\lblt}[1]{%
\hypersetup{linkcolor=black}%
\hyperref[tad:#1]{\ensuremath{\mathcal{I}_{#1}^{(1)}}}%
\hypersetup{linkcolor=blue}%
}
\newcommand{\Lblt}[1]{%
\hypersetup{linkcolor=black}%
\hyperref[tad:#1]{\ensuremath{\mathcal{I}_{#1}^{(1),\xi=0}}}%
\hypersetup{linkcolor=blue}%
}
\newcommand{\TadL}[1]{\ensuremath{T_{#1}^{\xi=0}}}

\newcommand{\tblt}[2]{\hline\lblt{#1} & \igtad[#1][#2] & \restad[#1]}
% \newcommand{\lbls}[1]{$\mathcal{I}_{#1}^{(2)}$}

\newcommand{\lbls}[1]{%
\hypersetup{linkcolor=black}%
\hyperref[se:#1]{\ensuremath{\mathcal{I}_{#1}^{(2)}}}%
\hypersetup{linkcolor=blue}%
}
\newcommand{\tbls}[1]{\hline\lbls{#1} & \igself[#1] & \resself[#1]}
\newcommand{\cpl}[2]{\ifthenelse{\isempty{#2}}{\mathtt{#1}}{\mathtt{#1}[\scalebox{.8}{$#2$}]}}
\newcommand{\m}{\textsl{\texttt{m}}}
\newcommand{\tI}[3]{%
  \ifthenelse{\isempty{#2}}{%
    \ifthenelse{\isempty{#3}}{%
      t_{#1}%
      }{%
      t_{#1}{(\scalebox{.8}{$#3$})}
    }%
  }{%
    \ifthenelse{\isempty{#3}}{%
      t_{#1}^{(#2)}%
      }{%
      t_{#1}^{(#2)}{(\scalebox{.8}{$#3$})}%
    }%
  }%
}
\newcommand{\tIL}[3]{%
  \ifthenelse{\isempty{#2}}{%
    \ifthenelse{\isempty{#3}}{%
      t_{#1}^{\xi=0}%
      }{%
      t_{#1}^{\xi=0}{(\scalebox{.8}{$#3$})}
    }%
  }{%
    \ifthenelse{\isempty{#3}}{%
      t_{#1}^{(#2),\,\xi=0}%
      }{%
      t_{#1}^{(#2),\,\xi=0}{(\scalebox{.8}{$#3$})}%
    }%
  }%
}
\newcommand{\f}[3]{%
  \ifthenelse{\isempty{#2}}{%
    \ifthenelse{\isempty{#3}}{%
      f_{#1}%
      }{%
      f_{#1}{(\scalebox{.8}{$#3$})}
    }%
  }{%
    \ifthenelse{\isempty{#3}}{%
      f_{#1}^{(#2)}%
      }{%
      f_{#1}^{(#2)}{(\scalebox{.8}{$#3$})}%
    }%
  }%
}
\newcommand{\Real}[1]{\Re\hspace{-1pt}\mathfrak{e}{\left[#1\right]}}

\newcounter{notecount}
\setcounter{notecount}{1}
\newcommand{\note}[3]{\marginpar{\color{#3}$^{\arabic{notecount})}$}
    {\color{#3}\footnotesize
    [#1$_{\arabic{notecount}}$: #2]}%
  \addtocounter{notecount}{1}}%
\newcommand{\notemg}[1]{\note{mg}{#1}{blue}}
\newcommand{\notesp}[1]{\note{sp}{#1}{green}}


==> unicode.tex <==
\usepackage[utf8]{inputenc}
\newcommand{\unicodegamma}{^^f0^^9d^^9b^^be}
\newcommand{\unicodesubfive}{^^e2^^82^^85}
\newcommand{\unicodescriptO}{^^f0^^9d^^92^^aa}
\newcommand{\unicodeitalicg}{^^f0^^9d^^91^^94}
\newcommand{\unicodesuptwo}{^^c2^^b2}
\newcommand{\unicodesupfour}{^^e2^^81^^b4}
\newcommand{\unicodesupsix}{^^e2^^81^^b6}
\newcommand{\unicodesupeight}{^^e2^^81^^b8}
\newcommand{\unicodePi}{^^f0^^9d^^9a^^b7}
\newcommand{\unicodecircumflex}{^^cb^^86}

